Augmenting Static Visualizations with PapARVis Designer

This paper presents an authoring environment for augmenting static visualizations with virtual content in augmented reality. Augmenting static visualizations can leverage the best of both physical and digital worlds, but its creation currently involves different tools and devices, without any means to explicitly design and debug both static and virtual content simultaneously. To address these issues, we design an environment that seamlessly integrates all steps of a design and deployment workflow through its main features: i) an extension to Vega, ii) a preview, and iii) debug hints that facilitate valid combinations of static and augmented content. We inform our design through a design space with four ways to augment static visualizations. We demonstrate the expressiveness of our tool through examples, including books, posters, projections, wall-sized visualizations. A user study shows high user satisfaction of our environment and confirms that participants can create augmented visualizations in an average of 4.63 minutes.

==> tex/_deprecated/1-introduction-2.tex <==
\section{Introduction}

% Visualizations are widely used to present information in printed materials such as posters, textbooks and brochures, newspapers, or display boards. 
% Due to being extremely low-tech, using these media makes is very simple to create, distribute, view, and engage with the visualization content; visualizations can be exported as PNGs or SVGs using common creation editors such as Tableau, D3~\cite{Bostock2011} or more bespoke editing environments such as Data Illustrator~\cite{} or Charticulator~\ or projected visualizations does not require any specific hardware, it can happen situated (e.g., \textit{in} a building, \textit{at} an exhibition), viewers are usually free to engage with the visualization through touch, annotation, and sharing thoughts and discussion with others. 
Easy to create, view, and distribute, 
printed materials, such as posters, textbooks, or display boards, 
are widely used in real world to present data visualizations. 

Visualizations are widely used to present information 
in printed materials such as posters, textbooks and display boards. 

These visualizations can be created using common creation editors such as Tableau and D3~\cite{Bostock2011}. 
They can be viewed and distributed situated without requiring any specific hardware. 
Moreover, viewers can freely engage with them through touch and annotation.


However, one problem common to printed visualizations is that the visualizations are \textit{static}. 
The displayed information is limited in both \textit{space and time}. 
% Static visualizations are prone to being out-of-date, users cannot obtain additional details, and space might sometimes be limited (e.g., on posters). 
Because of limited space, visualization designers have to make careful choices of the data content and the visual encoding to fit a given layout such as a portrait magazine page, a dedicated area on a poster, or a long corridor wall (Figure XX). 
% Moreover, once new information or data is available, the visualization becomes outdated---and in the worst case---deceptive. 
Because of dynamic data, the visualization can easily become outdated---and in the worst case---deceptive once new information or data is available.

To address these issues, this paper presents an authoring environment---\tool{}---for designing static visualizations and augmenting them with virtual content in an integrated workflow. 
We employ Augmented Reality (AR) technique since it can provide an extra display layer that shows custom and personal information on-demand: \ben{detail some ideas of how AR can augment static visualizations: complementary visualization, more details, alternative ... }. 
In the past, AR has been used to augment physical documents with XX~\cite{} and 
 make printed visualizations interactive~\cite{visar}. 
 However a structured exploration of augmented static visualizations is still missing.
It is challenging for designers is to create \textit{consistent} (C2) representations (e.g., color values, styles, positions) of the visualization in both media, static and virtual, and to \textit{avoid obstruction, clutter, and misleading designs} (C3) of the original static visualization. 
 Moreover, few if any tools can explicitly design and debug both static and augmented content simultaneously. 
 The current design workflow typically includes tools for static visualizations, tools for augmented visualization such as Unity, DXR~\cite{}, IATK~\cite{}, and potentially frequentl switching between these tools due to the lack of \textit{integration} (C$_{hallenge}$1).
%  a fact we partially attribute to the tedious design process and missing set of convincing examples. For example, a design workflow includes tools for static visualizations, tools for augmented visualization such as Unity, DXR~\cite{}, IATK~\cite{} and potentially frequently switching between them due to the lack of \textit{integration} (C$_{hallenge}$1). A futher challenges is to create \textit{consistent} (C2) representations (e.g., color values, styles, positions) of the visualization in both media: static and virtual and to \textit{avoid obstrusion, clutter, and misleading designs} (C3) of the original static visualization. 
Our goal with \tool is to provide an integrated authoring environment that supports a seamless authoring process for design, debugging, and deployment.
 
% The design of \tool{} (Section XX) is based on a design space (Section XX), that defined four ways of how static and virtual content can be combined. 
The design of \tool{} (Section XX) is based on a design space (Section XX) that defines four types of combinations between static and virtual content. 
As DXR has been proven useful in the past~\cite{Sicat2019}, \tool{} adapts similar approach, yet directly delivers an extension to the Vega grammar~\cite{Satyanarayan2016}, leveraging its simplicity and expressiveness to specify 2D visualizations.
\tool{} enable designers to create printed and 2D virtual visualizations based on the same specification
and to deploy the virtual visualization with one click.
Two bespoke features are included to facilitate the design process;
first, it provides a \textbf{preview} of the augmented paper visualization
that allows designers to view their designs on the desktop environment,
thus reducing switching between devices;
second, based on the design space, it \textbf{automatically verifies} the validity of a design and provides guidelines for correcting the design, ensuring consistency between the static and virtual visualizations.

To demonstrate the expressiveness of \tool{},
we provide an exemplary gallery of 
13 augmented paper visualizations (Figure 1), each varying in
\textbf{data type} (\emph{e.g.}, tabular, hierarchical, network, and geo-spatial),
\textbf{chart type} (\emph{e.g.}, node-link, matrix, sunburst, trajectory, ridgeline plot, and box plot),
\textbf{media} (\emph{e.g.}, poster, name card, map, resume, leaflet, book, newspaper, and wall printing),
and \textbf{purpose} (\emph{e.g.}, showing new, more, and personal data).
A controlled user study with 12 visualization designers who have no AR development experience suggests the overall usability of \tool{}.
All participants could successfully create and augment paper visualizations in an average of 4.75 minutes.
We also found the proposed two features (preview and automatic verification) were indispensable for their creation workflow.

In summary, the contribution of this paper is threefold: \textit{1)} a structured design space for augmenting static visualizations, 
\textit{2)} an authoring environment \qianwen{that enables the creation of both printed and 2D virtual visualization in an integrated workflow}, 
and 
\textit{3)} an evaluation consists of an exemplary gallery and a controlled user study.
\ben{make sure intro finishes with 1st column, max.}


==> tex/_deprecated/1-introduction-3.tex <==
\newpage
\section{Introduction}

Data visualizations---in the form of posters, in newspapers, journals, scientific reports, on public displays as well as slideshows and mobile screens---become increasingly more widespread. 
%Visualizations are widely available and distributed as printed material such as posters, in textbooks, brochures, and newspapers, or on display boards. 
In most of these cases, visualizations are printed on paper, which, due to its extremely low-tech, makes it very simple to create, distribute, view, and engage with the visualization content: %; visualizations can be exported as PNGs or SVGs using common creation editors such as Tableau, D3~\cite{Bostock2011} or more bespoke editing environments such as Data Illustrator~\cite{} or Charticulator~\ or projected visualizations does not require any specific hardware, it can happen situated (e.g., \textit{in} a building, \textit{at} an exhibition), viewers are usually free to engage with the visualization through touch, annotation, and sharing thoughts and discussion with others. 
%Easy to create, view, and distribute, 
%printed materials, such as posters, textbooks, and display boards, 
%are widely used by peoples (\emph{e.g.}, designers, researchers, and journalism) 
%to present data visualizations. 
visualizations can be created using common creation editors 
such as Tableau and D3~\cite{Bostock2011}, 
or more bespoke editing environments such as Data Illustrator~\cite{Liu2018} or Charticulator~\cite{Ren2019};
they can be viewed in-situ without requiring any specific hardware; viewers can freely engage with them through touch, pen and annotation,
and sharing thoughts and discussions in collaborative settings. In short---it is becoming increasingly easy to create and distribute visualizations which in turn has lead to a significant amount of existing visualization graphics.

A significant problem with this way of distributing visualizations is that these visualizations are \textit{static}, \textit{i.e.}, the displayed information is limited in both \textit{space} and \textit{time}.
Because of limited display space, visualization designers have to make careful choices on the data content and the visual encoding to fit a given layout such as a portrait magazine page, a dedicated area on a poster, a mobile screen, or a long corridor wall (\autoref{fig:outdated-tl}b). 
Moreover, once new information or data is available, the visualization becomes outdated (limited in time)---and in the worst case---becomes deceptive. These characteristics make a large amount of the many printed visualizations inherently \textit{incomplete}, compared with digital ones.

%To address these issues, 
% this paper presents an authoring environment---\tool{}---for designing static visualizations and augmenting them with virtual content in an integrated workflow. 
%we employ 
Augmented Reality (AR) can provide a possible solution to limited static visualizations by adding an extra dynamic display layer 
that shows additional and custom information on-demand. This can be used to complement a visualization with additional data (\autoref{fig:outdated-tl}a), show details,
updating outdated data (\autoref{fig:outdated-tl}b), or highlight data (\autoref{fig:outdated-tl}c).
In the past, AR has been successfully used to augment physical documents~\cite{BillinghurstKP01} and 
to make static visualizations interactive~\cite{visar}. 
However, a structured exploration of augmenting static visualizations and how to support their creation is largely missing. Currently, a designer must use different tools for static visualizations, and for virtual visualizations~\cite{Sicat2019, Cordeil2019}, 
% potentially 
frequently switching between tools due to the lack of \textit{integration} (C1).
It is also challenging for designers to create \textit{consistent} (C2) representations (\textit{e.g.}, color values, styles, positions) 
of the visualization in both static and virtual, 
and to \textit{avoid obstruction, clutter, and misleading designs} (C3) of the static visualization. 
%  a fact we partially attribute to the tedious design process and missing set of convincing examples. 
% For example, a design workflow includes tools for static visualizations, tools for augmented visualization such as Unity, DXR~\cite{}, IATK~\cite{} and potentially frequently switching between them due to the lack of \textit{integration} (C$_{hallenge}$1). 
% A futher challenges is to create \textit{consistent} (C2) representations (e.g., color values, styles, positions) of the visualization in both media: static and virtual and to \textit{avoid obstrusion, clutter, and misleading designs} (C3) of the original static visualization. 
%No tool can explicitly design and debug 
%both static and virtual content simultaneously. 
%We aim to provide an integrated authoring environment that supports a seamless authoring process for design, debug, and deployment.
 
To address challenges C1-C3, this paper introduces \textit{\textbf{\tool{}}, an authoring environment for designing static visualizations and augmenting them with virtual content in an integrated workflow.} 
The design of \tool{} (Sec.\ref{sec:tool}) is based on a design space (Sec.\ref{sec:design_space}) 
that defines possible and valid ways of combining static and virtual content. 
Similar to DXR~\cite{Sicat2019}, 
\tool{} %adapts similar approach, yet directly 
delivers an extension to the Vega grammar~\cite{Satyanarayan2016},
leveraging its simplicity and expressiveness to specify 2D visualizations.
\tool{} enables designers to create static and 2D virtual visualizations 
based on the same specification
and to deploy everything with one click. To facilitate design and avoid invalid combinations, we included two bespoke features into \tool{}: first, \textbf{\feata{}} gives a preview of the augmented static visualization
that allows designers to view their designs on the desktop environment,
thus reducing switching between devices;
second, \textbf{\featb{}} automatically validates a design based on our design space and provides guidelines for correction to ensure consistency between the static and virtual visualizations.

To demonstrate the expressiveness of \tool{},
we provide an exemplary gallery of 
13 augmented static visualizations (\autoref{fig:outdated-tl} and \autoref{fig:gallery}), 
each varying in data type, 
%(\emph{e.g.}, tabular, hierarchical, network, and geo-spatial),
chart type, 
%(\emph{e.g.}, node-link, matrix, sunburst, trajectory, ridgeline plot, and box plot),
media, 
%(\emph{e.g.}, poster, name card, map, resume, leaflet, book, newspaper, and wall printing),
and purpose. 
%(\emph{e.g.}, showing new, more, and personal data).
A controlled user study with 12 visualization designers but without
further experience in AR development suggests the overall usability of \tool{} and the two main features \feata{} and \featb{}. \tool{} is available at \url{http://anonymized-for-review.com}.

%all participants could successfully create augmented static visualizations in an average of 4.63 minutes.
% We also found the proposed two features (\feata{} and \featb{}) 
% were indispensable for their creation workflow.

% In summary, the contribution of this paper is threefold: 
% \textit{1)} a structured design space for augmenting static visualizations, 
% \textit{2)} an authoring environment that enables the creation of both static and virtual visualizations in an integrated workflow, 
% and  \textit{3)} an evaluation consists of an exemplary gallery and a controlled user study.

% \ben{mention mobile vis for litle space}


==> tex/_deprecated/1-introduction.tex <==
\section{Introduction}
%%%%%
%% - A more convincing list of features of what exactly your tool is offering
%% - 1-2 sentences about the examples.
%% - ~2 sentences on what your study found
%%%%%%%%%

Visualization has been widely used to present information in printed materials,
such as posters, textbooks, and brochures.
However, 
a printed visualization is 
limited by space (\emph{i.e.}, the size of a printed canvas is restricted)
and time (\emph{i.e.}, the content on printed materials is fixed).
Due to these limitations, % of space and time,
designers usually have to 
omit the background details
if the canvas for visualization is insufficient
and recreate the whole design
if the latest information need to be presented.

%% 2. Why AR can handle this limitation
Emerging AR technology 
has the capability 
to break through the aforementioned two limitations.
By merging the reality and virtuality,
AR can 
visually enlarge the printed canvas for additional data
and repeatedly fetch the datasource for updated data,
%display the latest data in real time,
% printed visualization for display the latest data in real time
thereby extending printed visualizations spatially and temporarily.
Furthermore,
by digitizing the printed content, %% materials with the capability of digitization,
AR can augment the capability of a static visualization, \emph{e.g.}, turns it into an interactive or animated visualization.
% rather than extending the content on it.

Previous explorations on 
augmenting printed visualizations are still scarce.
On one hand,
AR has been employed
to augment general physical documents
(\emph{e.g.}, providing additional details~\cite{BillinghurstKP01} 
and allowing words loop up~\cite{Li2019})
rather than visualizations.
On the other hand,
researchers have investigated
visualizing data in AR environments~\cite{Bach2018, Butscher2018},
instead of augmenting printed visualizations through AR.
In this study,
we explore augmenting printed visualizations
with virtual content through AR.
Specifically,
as a first step,
we focus on virtual content that is 
1) \emph{2D}, 2) \emph{static}, and 3) \emph{data visualization}.
We aim to tackle the problem of 
\cmo{\emph{how to enable designers to create augmented paper visualizations}}.

% Crafting 2D AR visualizations 
% to augment printed visualizations is not an easy task.
Crafting augmented paper visualizations is not an easy task,
requiring the designer to create both 
the reality (\emph{i.e.}, printed visualizations) 
and the virtuality (\emph{i.e.}, virtual visualizations in AR). 
The primary challenges are implied by the following requirements:
\begin{itemize}
    \item \textit{2D in AR}.
    Existing tools (\emph{e.g},~\cite{Sicat2019, Cordeil2019}) 
    for creating virtual visualizations in AR 
    mainly focus on 3D visualizations,
    thus requiring knowledge of 3D computer graphics 
    (\emph{e.g.}, shader and 3D camera)
    and do not support 2D visualizations well
    (\emph{e.g.}, cannot create circular charts and tree diagram).
    A tool for creating 2D visualizations in AR is required.

    \item \textit{Consistent}.
    Augmenting a printed visualization 
    with a virtual visualization requires
    a high consistency in the data, visual styles, and positions
    between the printed and virtual visualization.
    Otherwise, the mismatch may lead to confusion and misleading
    in reading the augmented paper visualization.
    A tool to help designers ensure 
    the consistency %and alignment 
    between the printed and virtual visualization is required.
    
    \item \textit{Unobtrusive}.
    A typical workflow to create augmented paper visualizations
    starts from creating a 2D visualization $V_r$ for printing,
    % (\emph{e.g.}, using Vega~\cite{Satyanarayan2016}]),
    followed by creating an virtual visualization $V_v$,
    % (\emph{e.g.}, using DxR~\cite{Sicat2019}),
    and finished with developing an AR system 
    to recognize $V_r$ and register $V_v$.
    In this workflow, the designer 
    % This workflow requires 
    frequently switch between tools and devices,
    thus requiring    
    % Using existing tools to create augmented paper visualizations
    a significant amount of efforts
    and dedicated programming skills.
    An tool that supports an unobtrusive workflow is required.

\end{itemize}

To tackle these challenges, % and inform our authoring environment,
we first systematically study 
the design space of augmenting printed visualizations,
which outlines four methods %as well as their extending point and validity
to augment printed visualizations through AR.
Based on the design space,
we design and implement \tool{}, an authoring environment,
for creating augmented paper visualizations.
By employing an browser/server architecture,
% By separating the design and deployment of visualizations,
\tool{} separates the design and deployment of visualizations,
thus allowing designers to focus on the visualization design
and get rid of the AR deployment.
\tool{} extends Vega, 
an declarative visualization grammar,
to leverage the simplicity and expressiveness of Vega on creating 2D visualizations (\cmo{2D in AR}).
A designer can create printed visualizations as well as 
2D virtual visualizations based on the same specification (\cmo{consistent})
% how the virtual visualization will augment the printed visualization in \tool{}
and deploy the virtual visualization to AR environments in one click (\cmo{unobtrusive}).
\tool{} includes two advanced features to facilitate the design process:
1) it provides a preview of the augmented paper visualization
that allows designers to view their design on the desktop environment,
thus reducing the switching between devices (\cmo{unobtrusive});
and 2) it automatically verifies 
whether a design violates the design space
and provide guidelines for correcting the design,
thus ensuring the data consistency between the printed and virtual visualization (\cmo{consistent}).

To demonstrate the expressivity of \tool{},
we provide an exemplary gallery of 
13 augmented paper visualizations varying in
data type (\emph{e.g.}, tabular, hierarchical, network, and geo),
chart type (\emph{e.g.}, node-link, matrix, sunburst, trajectory, ridgeline plot, and box plot),
paper media (\emph{e.g.}, poster, name card, map, resume, leaflet, book, newspaper, and wall printing),
and purpose (\emph{e.g.}, show new, show more, and show personal).
A controlled user study with 12 designers who have no AR expertise
is conducted to evaluate the usability of \tool{} 
as well as the usefulness of its two advanced features.
Results suggest that participants 
can successfully create augmented paper visualizations
in an average of 4.75 minutes
and the two features are indispensable for creating augmented paper visualizations.

The contributions are threefold: 1) a structured design space for augmenting printed visualizations, 2) an authoring environment, 
and 3) an evaluation consisits of an examplar gallery and a controlled user study.

==> tex/_deprecated/2-related_bk.tex <==
\section{Related Work}

This section overviews prior studies 
on AR visualization,
augmenting physical documents,
and visualization authoring tool.

\subsection{AR Visualization}
AR allows combining the virtuality with the reality,
thereby enhancing the connection between 
the digital data and the physical world.
Willett et al.~\cite{Willett2017} 
formalized the conceptual framework 
of embedded data representations
to unify the research on 
visualization systems that connect to the physical world.
Their framework provide guidelines
of using AR to integrate data with the physical world.

Many benefits of visualizing data in AR have been reported by previous research.
For example, AR can facilitate certain visual explorations and collaborative analysis.
By comparing users' performances in interactive explorations
in a head-mounted display (HMD) AR, mobile AR, and desktop environment,
Bach et al.~\cite{Bach2018} reported that 
the HMD AR environment with tangible markers
is more effective for tasks 
requiring spatial perception and high degree-of-freedom interactions.
Butscher et al.~\cite{Butscher2018} presented ART,
an AR collaborative analysis tool, 
and reported that ART can facilitate communication and coordination between collaborators since the interaction is grounded in the physical world.
%% 
Besides, 
AR can visualize data closer to its physical referents,
enabling situated analytics.
Zhao et al.~\cite{sa-ego-centric} 
developed an mobile AR system to 
support on-site analysis of co-authoring patterns of researchers.
SiteLens~\cite{White2009} visualizes relevant data
in the 3D physical context for urban site visits.
ElSayed et al.~\cite{ElSayed2015}
developed an AR system to help customers 
filtering, finding, and ranking products during shopping. 
Moreover, AR have been used to present 
visualizations for communication purposes~\cite{Chen2019}
as AR can better engage the users.

In summary,
through visualizing data with the physical world,
previous work shows that AR
can connect the virtual data to the physical space,
augment the real world with rich virtual content,
and even engage and motivate users.
We draws on this line of work 
and attempts to augment printed visualization 
with virtual visualization,
harnessing the best of both physical and digital worlds. 

% With a recent surge in the popularity of HMD (\emph{e.g.}, HoloLens),
% researchers have attempted to 
% explore visual analytics
% in HMD AR environments.

% However, current HMD devices have various deficiencies, 
% including narrow field-of-view, low resolution, 
% and inaccurate tracking~\cite{Baumeister2017}.
% In addition,
% users needed more time to become familiar with the HMD devices~\cite{Bach2018},
% which are still relatively new to most consumers.

% As another type of AR devices, 
% mobile devices are more familiar to the masses.
% Several research based on mobile AR 
% have been presented for various applications.
% MelissAR~\cite{ia-mobile-bee}, 
% a tablet AR system, 
% shows drift information in-situ 
% to assist beekeepers in understanding bee behaviors.
% Existing work mainly focuses on
% visualizing data in AR % environments
% while we aim to using AR to
% augment printed visualizations.

\subsection{Augmenting Physical Documents}

A variety of AR systems 
(\emph{e.g.}, projector-based~\cite{Wellner91}, handeld-based~\cite{BillinghurstKP01}, and HMD-based~\cite{Li2019}) have been proposed 
to augment physical documents 
by providing additional functionality and content.
For example, HoloDoc~\cite{Li2019},
a mixed reality system based on HoloLens,
augments physical artifacts to 
allow users to take notes and look up words.
Although these systems 
augment physical documents with rich virtual content,
they are not designed for augmenting printed visualizations,
which requires a high level of 
information integrity,
visual style consistency,
and spatial alignment
between the printed and the virtual content.
Recently, initial explorations have been made 
to augment visualizations. 
Kim et al.~\cite{visar} presented VisAR,
an AR prototype system that 
provides interactive functions to static visualizations.
Differently,
we aim to use AR to extend printed visualizations
by providing additional information.

% However,
% the authors focused on the interactions
% rather than the design of augmenting static visualizations.
% 
% whereas the physical objects
% we are interested in are printed visualizations,
% which add unique constraints 
% to the design of virtual visualizations.
% To the best of our knowledge,
% no structured exploration of 
% augmenting printed visualizations exists.


% three levels alignments: 1. semantically, 2. visual styles I mean, 3. spatially
% \qianwen{"Printed visualization, as a special type of physical document, requires a high level of information consistency and a strict alignment "}  
% For example, Affinity Lens~\cite{Subramonyam2019} provides quantitative insights overlaid on physical notes, thus helping users to organize physical notes and summarize insights. 
% However, "say how vis is different from doc and why previous tools may fail" 
% “requires a high level of information consistency and strict alignment between the old and the updated visualization? I don't know, maybe” ""}

% Many previous projects augmented physical documents 
% to provide additional functionality (\emph{e.g.}, take notes and words look up) and content by using AR systems,
% including  (\emph{e.g.}, DigitalDesk~\cite{Wellner91}),
% handheld-based (\emph{e.g.}, MagicBook~\cite{BillinghurstKP01} and Affinity Lens~\cite{Subramonyam2019}),
% and HMD-based (\emph{e.g.}, HoloDoc~\cite{Li2019}).
% Although these systems 
% augment physical documents with rich virtual content,
% they are not designed for visualizations.

% used stationary projector to augment physical documents
% by providing 
% In recent years, 
%  and  AR have also been explored.
% Billinghurst et al.~\cite{BillinghurstKP01} 
% presented MagicBook
% that displays 3D scenes around the book pages
% through a handheld display.
% % Similarly, the Mixed Reality Book~\cite{GrassetDSB07}
% % symbiotically merged the physical pages
% % and virtual content when the book pages
% % are viewed through a handheld display.
% % With mobile AR,
% % Feng et al.~\cite{FengYX17}
% % proposed MagicToon that allows children 
% % to view their own 2D cartoon drawings on paper in 3D scenes.
% Affinity Lens, 
% proposed by Subramonyam et al.~\cite{},
% augments physical Affinity Diagramming using
% mobile AR to provides just-in-time quantitative insights overlaid on
% physical notes.
% Recently, Li et al.~\cite{Li2019} employed
% introduced HoloDoc,
% a mixed reality system based on HoloLens
% that augments physical artifacts 
% with rich interaction 
% and virtual content.

\subsection{Visualization Authoring Tool}

% Researchers have developed authoring tools
% to enable creating visualizations 
% for desktop and immersive environments.
A number of authoring tools have been proposed 
to facilitate the creation of visualization 
in desktop and AR environments.

%% Desktop
Prior work on creating desktop visualization
ranges from highly expressive programming toolkits
to easy-to-use WIMP UI tools.
Programming toolkits 
(\emph{e.g.}, D3~\cite{Bostock2011}, ProtoVis~\cite{})
provide strong expressiveness and 
support flexible visualization designs
but require a high level of programming skills.
Instead,
WIMP UI systems 
(\emph{e.g.}, Lyra~\cite{}, iVisDesigner~\cite{Ren2014}, and Voyager~\cite{Wongsuphasawat2016})
lower the barrier of creating visualizations 
by providing interactive functions
to allow users to design visualizations via drag and drop,
but compromising the flexibility.
To strike a balance between expressivity and simplicity,
Vega~\cite{Satyanarayan2016} and Vega-Lite~\cite{Satyanarayan2018}
enable users to define visualization 
with concise declarative specification in JSON format.
% These systems usually
% Recently,
% researchers have developed pen- and touch-based tools
% (\emph{e.g.}, ivolver~\cite{Mendez2016}, DataInk~\cite{Xia2018}, and DataToon~\cite{Kim2019})
% to support creativity design 
% by harnessing the human directed manipulation skills.
Overall, these systems 
focus on 2D visualizations on desktop platforms
but cannot create visualizations in AR.

Recently,
several tools have been proposed
for creating visualization in AR environments.
For examples,
MARVisT~\cite{Chen2019},
a touch-based creativity support tool,
% that extracts the information from reality 
was proposed to assist general users in creating AR glyph-based
visualizations.
Besides,
programmatic toolkits have presented to support more flexible visualizations.
Sicat et al.~\cite{Sicat2019} presented DXR,
a fast prototyping toolkit based on Unity, 
that provides both programmatic 
and graphical user interfaces 
to help designers create immersive visualizations.
IATK~\cite{Cordeil2019},
another toolkit package for Unity,
allows interactive authoring of data visualisation for immersive analytic.
% Although these systems allow creating 
% diverse 3D visualizations in AR environments,
These systems mainly focus on 3D visualizations 
and do not support 2D visualizations well 
(\emph{e.g.}, cannot create circular charts and tree diagram).

However, the aforementioned tools are not suitable for creating augmented paper visualizations.
First,
none of these tools can create 2D visualizations
for both printing and displaying in AR,
thus requiring the designer to frequently
switch between tools.
Second, 
none of these tools can help designer to ensure
the consistency of data, visual styles, and positions
between the printed and the virtual visualization.
In this regard, 
we contribute an authoring environment 
to create visualization crossing between the reality and virtuality.


% they are not suitable to fulfill our goal,
% which requires creating 
% to augment printed visualizations.
% These tools focus on creating
% 3D visualizations in immersive environments,
% thus 
% They mainly support
% creating axis-based and glyph-based visualizations
% and fall short of others (\emph{e.g.}, circular charts, tree diagram, and network diagrams \cmo{double check}).
%% how to align
% \cmo{(ps:
% 2D tools: create 2d in desktop;
% immersive tools: create 3d in AR;
% ours: create 2d (but with more constraints) in AR;
% )}


% creating visualization that can both be printed on papers
% and displayed in AR.
% On one hand, the tools for desktop visualization
% cannot create visualization in AR

% these tools do not support
% creating  virtual  visualization  that  can  be  displayed  in  AR.

% allow creating diverse desktop visualization

% Although we also aim for creating visualizations,
% these system, however, are not suitable

% which
% The tools mentioned above 
% are developed for 
% either 2D visualization on desktop platforms
% or 3D visualization in immersive environments.


==> tex/_deprecated/3-design.tex <==
\section{Design Space}
\label{sec:design_space}

This section first discusses the difference between static visualizations
and augmented static visualizations and 
proposes a model for augmenting static visualizations, then it explores the design space under this model, and eventually summarizes a derived set of design goals for our authoring environment.

\subsection{What kind of augmented static visualizations is valid?}
\label{ssec:model}
In this work,
we distinguish between these three terms:
\textit{i.} \textit{static visualizations}~\inlinefig{figures/icon_vr}, which are static but can be in different media (\emph{e.g.}, be printed, projected, and displayed in digital screens),
\textit{ii.} \textit{virtual visualizations}~\inlinefig{figures/icon_vv}, which are displayed in AR 
(\emph{e.g.}, the virtual timeline in \autoref{fig:outdated-tl}b),
and \textit{iii.} \textit{augmented static visualizations}~\inlinefig{figures/icon_var}, which combine both static and virtual visualizations in AR.
\inlinefig{figures/icon_var} are different from \inlinefig{figures/icon_vr}
in two major aspects:
1) for designers, 
creating an \inlinefig{figures/icon_var}
requires creating both \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv};
% the static visualization  and the virtual visualization ;
% 2) for audiences,
% viewing an augmented visualization
% is similar to using a magic lens 
% to switch from $V_r$ to a view $V_{AR}$ that combines $V_r$ and $V_v$:
2) for audiences,
viewing an 
% augmented static visualization 
\inlinefig{figures/icon_var}
requires the switching between \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_var}:
\begin{equation}
    \inlinefig{figures/icon_vr} \rightarrow \inlinefig{figures/icon_var} = combine(\inlinefig{figures/icon_vr}, ~\inlinefig{figures/icon_vv})
    \label{eq:combineVR}
\end{equation}
Thus,
the creation of \inlinefig{figures/icon_var}
should integrate both \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv}
to avoid interrupting the designer.
Besides, the design of \inlinefig{figures/icon_var}
should ensure
that the switching between \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_var}
will not confuse and mislead the audience.

To maintain the perceptual effectiveness,
we propose that after switching to \inlinefig{figures/icon_var},
all the information of \inlinefig{figures/icon_vr} should remain;
thus the user can still easily perceive the old information
and trace what new data has been added through \inlinefig{figures/icon_vv}~\cite{eyesbeat}.
Specifically,
a valid \inlinefig{figures/icon_var} should be able 
to be described by the following model:
\begin{equation}
    \inlinefig{figures/icon_var} = \inlinefig{figures/icon_vr}~\oplus~\inlinefig{figures/icon_vv},
    \label{eq:principle}
\end{equation}
wherein the $\oplus$ means \textit{visually composite}, a subset of the
% \keepvalues
% \setlength{\intextsep}{0pt}%
% \setlength{\columnsep}{7pt}%
% \begin{wrapfigure}{r}{0.1\textwidth}
% 	\centering
% 	\includegraphics[width=0.1\textwidth]{figures/pie.png}
% \end{wrapfigure}
% \restorevalues
$combine$ 
in~\autoref{eq:combineVR}.
Intuitively,
this  model requires~\inlinefig{figures/icon_vv} not
to hinder the perception of~\inlinefig{figures/icon_vr},
\emph{e.g.}, interfering~\inlinefig{figures/icon_vr}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/traning}
    \caption{The validity of augmented static visualizations: a) A valid augmented bar chart; b) An invalid augmented pie chart.
    }
    \vspace{-2mm}
    \label{fig:training}
\end{figure}

For example, \autoref{fig:training} demonstrates when augmenting a dataset with more data items, the bar chart design is valid while the 
virtual pie chart interferes
the perception of the static pie chart.
We consider an~\inlinefig{figures/icon_var} as invalid 
if it does not follow the model in \autoref{eq:principle}.


\subsection{How can a static visualization be augmented by AR?}
\label{ssec:augmentations}

Based on the model (\autoref{eq:principle}),
the augmentation of a 
static visualization
\inlinefig{figures/icon_vr}
is determined by two dimensions: 
\textit{i.} the virtual visualization~\inlinefig{figures/icon_vv},
which can have \textbf{different} or the \textbf{same} visual encodings 
of \inlinefig{figures/icon_vr},
and \textit{ii.} visual composition $\oplus$,
which can combine \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} 
as an \textbf{integrated} view or two \textbf{separate} views.
We use these two dimensions to construct a design space (\autoref{fig:augmentations}), 
which outlines four ways to augment a \inlinefig{figures/icon_vr}:

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/augmentations}
    \caption{Four ways to augment static visualizations using AR: 
        a) Extended View;
        b) Composite View;
        c) Small Multiple;
        d) Multiple View.
    }
    \label{fig:augmentations}
\end{figure}

\begin{itemize}[noitemsep]
    \item \textbf{Extended View.}
    \autoref{fig:augmentations}a presents the scenario 
    that \inlinefig{figures/icon_vv} has the same visual encodings with \inlinefig{figures/icon_vr}
    and is integrated with \inlinefig{figures/icon_vr} in a single view. 
    \textit{\underline{Augmentation Point}}:
    In this augmentation method,
    \inlinefig{figures/icon_vv} and \inlinefig{figures/icon_vr} are actually the same visualization (\emph{i.e.}, use the same visual encodings in the same view) but different in data.
    The designer can extend \inlinefig{figures/icon_vr} with additional data,
    allowing a static visualization 
    to present continually updated data 
    or to provide details on demand.
    \textit{\underline{Validity}}:
    A particular validation point of this method
    is that the designer should consider the data dependency between \inlinefig{figures/icon_vr}
    and \inlinefig{figures/icon_vv}.
    Not all \inlinefig{figures/icon_vr} can be augmented in this way.
    For example, 
    a pie chart 
    % $V_r^{pie}$ 
    \biginlinefig{figures/icon_vrpie} 
    cannot be augmented with more data items through 
    % $V_v^{pie}$.
    \biginlinefig{figures/icon_vvpie}
    Specifically,
    \biginlinefig{figures/icon_vvpie}
    can only match the ``updated'' 
    % $V_r^{pie}$ % by appending new data items,
    \biginlinefig{figures/icon_vrpie}
    but not \biginlinefig{figures/icon_vrpie} itself.
    Thus, \biginlinefig{figures/icon_vvpie} will hinder the perception of \biginlinefig{figures/icon_vrpie}.
    In other words, 
    using this method, the designer must ensure 
    \inlinefig{figures/icon_vr} will not change when the new data is appended.
    
    \item \textbf{Composite View.}
    \autoref{fig:augmentations}b depicts the condition when 
    \inlinefig{figures/icon_vv} has different visual encodings with \inlinefig{figures/icon_vr} 
    and is integrated with \inlinefig{figures/icon_vv}.
    \textit{\underline{Augmentation Point}}:
    When augmenting \inlinefig{figures/icon_vr} in this way,
    the designer can visualize another dataset using \inlinefig{figures/icon_vv}
    that complements \inlinefig{figures/icon_vr},
    or can present extra data attributes of the dataset of \inlinefig{figures/icon_vr}.
    % that have not been visualized.
    \textit{\underline{Validity}}:
    Given \inlinefig{figures/icon_vv} 
    has different visual encodings from \inlinefig{figures/icon_vr},
    the designer does not need to concern the data dependency between
    them and should focus on general design issues, \emph{e.g.}, occlusions between \inlinefig{figures/icon_vv} and \inlinefig{figures/icon_vr}.
    
    % will not alter $V_r$.
    % that will not affect $V_r$.
    % the augmentation will always be valid 
    % (\cmo{I mean the designer only need to consider how to design a good vis and does not need to pay additional efforts on the validity of augmented paper vis.})

    \item \textbf{Small Multiple.}
    \autoref{fig:augmentations}c 
    shows the scenario where \inlinefig{figures/icon_vv} has the same visual encodings with \inlinefig{figures/icon_vr} 
    and is displayed as a separate view.
    \textit{\underline{Augmentation Point}}:
    % By this way,
    \inlinefig{figures/icon_vv} can be used to present other datasets in the same visual encodings of \inlinefig{figures/icon_vr}.
    Generally, the result of this method is a small multiple.
    \textit{\underline{Validity}}:
    The augmentation will always be valid as
    \inlinefig{figures/icon_vv} is displayed separately from \inlinefig{figures/icon_vr}.
    % (\emph{i.e.}, no direct visual interactions).
    However, since both \inlinefig{figures/icon_vv} and \inlinefig{figures/icon_vr} use the same visual encodings,
    the designers should consider whether the visual encodings fits for various datasets, \emph{i.e.}, the scalability issue.

    \item \textbf{Multiple View.}
    \autoref{fig:augmentations}d demonstrates the case 
    that \inlinefig{figures/icon_vv} 
    has different visual encodings with \inlinefig{figures/icon_vr}
    and is displayed separately from \inlinefig{figures/icon_vr}.
    \textit{\underline{Augmentation Point}}:
    Choosing this augmentation
    allows the designer to use AR to 
    extend \inlinefig{figures/icon_vr} 
    to a multiple view (\emph{e.g.}, a dashboard),
    presenting different perspective of the data behind \inlinefig{figures/icon_vr},
    or use \inlinefig{figures/icon_vv} 
    to visualize new datasets along with \inlinefig{figures/icon_vr} 
    that yields deeper insights into the data.
    \textit{\underline{Validity}}:
    This method can always ensure valid AR visualizations
    and has the most flexibility 
    as \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} are completely independent (both in data and visually).
    
\end{itemize}

In summary,
in our model,
a \inlinefig{figures/icon_vr} can be augmented 
in four different ways
with different augmentation points.
Among these four augmentation methods,
\textit{Extended View} is the most strict one,
as in which \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} 
are highly correlated;
\textit{Multiple View} is the most flexible one,
as in which \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} 
are completely independent of each other.

\subsection{Design Goals}
To create augmented static visualization \inlinefig{figures/icon_var},
we conceive our authoring environment to accomplish three main goals:

\textbf{G1: Integrate the workflow in one tool}---As mentioned in Sec.\ref{ssec:model},
to create a \inlinefig{figures/icon_var},
the designer is required to create both
the static \inlinefig{figures/icon_vr} and virtual \inlinefig{figures/icon_vv} visualization.
%However, as far as we know, no tools support both, thus requiring designers to frequently switch between tools (\emph{e.g.}, D3 \emph{vs}. DXR).
%This workflow requires a significant amount of efforts  and dedicated programming skills,
%and more importantly, 
%cannot support the design and debug both \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} concurrently.
We aim to integrate all steps of the workflow 
and allow designers without AR expertise
to create both \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} in a tool simultaneously: create the static visualization, create the virtual visualization, integrate both, test and debug, and deploy.

% \textbf{G2.Preview the AR visualization to avoid switching between devices.}
% \qianwen{G2:avoiding attention switching}
% \textbf{G2.Preview the visualization in one device.}
% \textbf{G2.Avoid the switching devices.}
\textbf{G2: Create the design in one platform}---Creating \inlinefig{figures/icon_var} may require the designer 
to work back-and-forth between the desktop platform and AR devices (e.g., head-mounted displays, mobile handheld).
This kind of offline workflow is tedious and time-consuming.
The authoring environment should alleviate this burden as much as possible.
Given that \inlinefig{figures/icon_vr} will be part of the reality,
we can preview the \inlinefig{figures/icon_vv} 
together with the \inlinefig{figures/icon_vr}
on the desktop platform to simulate the AR scenario,
thereby reducing the attention switching.
Moreover, some augmentations (\emph{e.g.}, \textit{Composite View}) 
may display data that is unknown during the creation,
\emph{e.g.}, future data. % to be obtained in the future.
Our authoring environment should allow previewing the \inlinefig{figures/icon_var}
no matter the data of the \inlinefig{figures/icon_vv} is certain or uncertain.

% \textbf{G3.Provide hints to facilitate the creation of valid augmented visualizations.}
% \qianwen{G3: validating the augmented visualization.}
% \textbf{G3.Validate the design in automated manner.}
% \textbf{G3.Avoid the manual validation.}
\textbf{G3: Provide automatic design support}---Our model describes how a \inlinefig{figures/icon_var} is valid.
As indicated by our design space, 
designing valid \textit{Extended View} is the most challenging
since in which there are data dependencies exist between the \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv}.
When new data is appended and visualized by the \inlinefig{figures/icon_vv},
a mismatch between the \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} can easily happen
due to inappropriate visual encodings,
leading to an invalid \inlinefig{figures/icon_var}.
When the data is large, or the visual encodings are complex, 
it will be difficult for the designer 
to verify and debug the inappropriate design manually.
Thus, the authoring environment should
automatically verify the design
and provide hints for debugging inappropriate visual encodings.


==> tex/_deprecated/5-tool.tex <==


\section{PAPARVIS DESIGNER}
\label{sec:tool}

This section describes the design and implementation of \tool{}, 
our authoring environment for augmented static visualizations.

\subsection{Workflow}

\begin{figure}[thb]
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/workflow}
    \caption{A workflow creates both static and virtual visualizations.}
    \label{fig:workflow}
\end{figure}

% To fulfil G1,
% the tool should be able to create both static \inlinefig{figures/icon_vr} 
% and virtual \inlinefig{figures/icon_vv} visualizations.
\tool{} creates both static and virtual visualizations.
Instead of developing a tool that combines both
the functionalities of visualization tools
for desktop and AR environments,
we abstract the common part of them
and propose a decoupled workflow (\autoref{fig:workflow}).
By separating the specification
(\emph{i.e.}, designing visualizations) 
from the deployment
(\emph{i.e.}, presenting visualizations),
our workflow allows designers without AR expertise 
to create both $V_s$ and $V_v$ (G1)
in some well-established authoring tools
and leave the AR deployment to AR experts.

Specifically, 
our workflow adopts a browser/server architecture.
In the workflow, 
the designer uses a \inlinefig{figures/icon_vis}
to create a ``stem'' visualization~\inlinefig{figures/icon_v},
which can then be captured as a \inlinefig{figures/icon_vr}.
While the \inlinefig{figures/icon_vr} is static,
the designer can continue updating \inlinefig{figures/icon_v},
similar to update a web page,
and use a converter~\inlinefig{figures/icon_converter} 
to convert it into a \inlinefig{figures/icon_vv}.
An AR viewer can be used to recognize the \inlinefig{figures/icon_vr}
and register the \inlinefig{figures/icon_vv}
to obtain the \inlinefig{figures/icon_var}.
By this mean, both \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv}
are created based on the same specification,
thus maintaining a high level of consistency.

We implement the workflow in \tool{} (\autoref{fig:pipeline}),
which consists of three main components: % corresponding to the
\begin{itemize}[noitemsep]
    \item \textbf{VegaAR Editor} is built based on Vega Editor~\cite{vegaEditor},
    a UI editor of Vega.
    % Vega is a popular declarative grammar 
    % for specifying data visualizations in JSON format,
    % which strike a good balance between the simplicity and expressivity.
    In VegaAR Editor,
    the designer can create a \inlinefig{figures/icon_vr} 
    following the same practice in Vega
    and specify the \inlinefig{figures/icon_vv}
    in an \texttt{ar} block,
    which will be further introduced in the next section (Sec.\ref{ssec:preview}).
    When finishing the creation,
    the designer can \texttt{publish} the design
    to export the \inlinefig{figures/icon_vr} (\autoref{fig:pipeline}d)
    and push the whole specification, including the \texttt{ar} block,
    to a \textit{SpecHub}.
    VegaAR Editor will generate a QRCode that contains the unique identity
    of the \inlinefig{figures/icon_vr} that links to the specification on SpecHub.

    \item \textbf{SpecHub} is deployed on a cloud server 
    to receive and host the specifications from VegaAR Editor.
    Besides,
    it prepares all prerequisites for the \inlinefig{figures/icon_var},
    such as processing the specification of \inlinefig{figures/icon_vr} 
    to generate the AR reference image so that \inlinefig{figures/icon_vr} 
    can be recognized by AR viewers,
    parsing the \texttt{ar} block to generate the \inlinefig{figures/icon_vv},
    hosting and returning the \inlinefig{figures/icon_vv} when it is fetched by AR viewers.
    
    \item \textbf{AR Viewer} is the endpoint (\emph{i.e.}, browser) 
    for audiences to view the \inlinefig{figures/icon_var}. 
    When scanning a \inlinefig{figures/icon_vr},
    an AR viewer will identify the \inlinefig{figures/icon_vv} based on its QRCode, 
    fetch its corresponding \inlinefig{figures/icon_vv} from the SpecHub,
    and register \inlinefig{figures/icon_vv} onto \inlinefig{figures/icon_vr}
    to present the \inlinefig{figures/icon_var} (\autoref{fig:pipeline}e).
    The AR viewer is not platform-specific.
    In this work, we have implemented three AR viewers
    on the iOS, Android, and web-based platform, respectively.
\end{itemize}

With this workflow, designers can easily create \inlinefig{figures/icon_var}
in one tool without digging into the AR details.

\subsection{AR-Preview}
\label{ssec:preview}

We design \feata{} to avoid the frequently switching between devices (G2).
Specifically,
to preview the \inlinefig{figures/icon_vv} together with \inlinefig{figures/icon_vr},
the designer must explicitly specify the \inlinefig{figures/icon_vv} during the creation,
which is not supported by the current Vega grammar.
Thus, we extend the Vega grammar
by adding an additional configuration block \texttt{ar} (\autoref{fig:pipeline}a) to it.
The \texttt{ar} block is optional in a specification
and will not affect the \inlinefig{figures/icon_vr}.
In the \texttt{ar} block,
the designer can explicitly specify the augmentation method,
the visual encoding,
and the data of a \inlinefig{figures/icon_vv},
no matter the data is certain or uncertain:
\begin{itemize}[noitemsep]
    \item \textbf{Certain}. 
    When the data is known
    (\emph{e.g.}, some detail information cannot be presented due the space limitation),
    the designer can specify the \inlinefig{figures/icon_vv} 
    in the \texttt{ar} block,
    starting from defining its 
    % how it will augment \inlinefig{figures/icon_vr} 
    % in one of the four 
    augmentation method:
    1) in \textit{Extended View},
    the designer only needs to specify 
    which datasets of \inlinefig{figures/icon_vr} will be appended with what data
    and can reuse other visual encodings of the \inlinefig{figures/icon_vr};
    % , rather than specifying the visual encoding of \inlinefig{figures/icon_vv};
    2) in \textit{Composite View}, 
    % in addition to appending data to the detests of \inlinefig{figures/icon_vr}, 
    the designer can specify a new visualization in the \texttt{ar} block
    with new datasets or with the existing datasets of \inlinefig{figures/icon_vr};
    3) in \textit{Small Multiple},
    the designer only need to specify the new datasets and the layout of the virtual small multiples in relation to the \inlinefig{figures/icon_vr};
    4) in \textit{Multiple View}, the designer is allowed to create a complete new visualization in the \texttt{ar} block 
    and define its placement with respect to the \inlinefig{figures/icon_vr}.

    \item \textbf{Uncertain}.
    The data of the \inlinefig{figures/icon_vv} could be uncertain during the creation 
    (\emph{e.g.}, the data can only be obtained in the future).
    In this case,
    it will be arduous for the designer to image the \inlinefig{figures/icon_vv}.
    We provide a \texttt{placeholder} mechanism to
    allow designers generate mockup data using wildcard.
    In the \texttt{ar} block, 
    the designer can create placeholder datasets
    and generate their data by 
    specifying the data type (\emph{e.g.}, categorical, temporal, and quantitative),
    number of datum,
    and ranges or potential options of the values
    of each column.
\end{itemize}

By explicitly defining the \inlinefig{figures/icon_vv} in the \texttt{ar} block,
VegaAR Editor will provide visual preview of the virtual content 
together with the \inlinefig{figures/icon_vr},
thus reducing the switching between devices.

\subsection{Validator}

An \textit{Extended View} (see design space) can easily be invalid
given the data dependency between \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} (\emph{e.g.}, the pie chart in Sec.\ref{ssec:model} and the tree diagram in Sec.\ref{sec:usage-scenario}).
When choosing this augmentation method,
\tool{} automatically verifies the dataflow of the visual design
and provides hints for debugging invalid visual encodings (G3).

\begin{figure}[thb]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/hint}
    \caption{Validate the visual design by comparing the dataflows, thus enabling providing debug messages specific to a transform.}
    \label{fig:dataflow}
\end{figure}

%% solution
Instead of using a rule-based method,
we propose to validate the visualization
by comparing the dataflow between \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_var}.
%% the process of visualization
A general visualization process of a dataset $D_r$
can be summarized in~\autoref{fig:dataflow}:
$D_r$ will first be processed by
a serials of data transforms
and then mapped to visual channels
to construct the \inlinefig{figures/icon_vr}.
%% when will be valid
As demonstrated in Sec.\ref{ssec:augmentations},
in a valid \inlinefig{figures/icon_var},
the \inlinefig{figures/icon_vr} should remain unchanged
after appending the new data $D_v$,
which means its all intermediate states $D_r^{T}$
before the visual mapping
should also be unchanged.
Thus,
for each data transform,
we can compare 
the intermediate state of \inlinefig{figures/icon_vr} 
and \inlinefig{figures/icon_var}
to see whether the intermediate state derived from $D_r$
is changed.
If an intermediate state is changed,
for example ${D'}_r^{T2} \neq D_r^{T2}$,
it means the transform (\emph{i.e.}, Transform$2$)
makes the \inlinefig{figures/icon_vr} changed after appending new data,
thus leading to an invalid \inlinefig{figures/icon_var}.
Therefore, 
we can give the designer a hint specific to a transform 
and further provide messages for fixing it (\emph{e.g.}, \autoref{fig:dataflow}a)
regardless of the complexity of the visualization. For example, when trying to overlay a treemap, the system warns \texttt{avoid 'treemap'  when new nodes are added to the internal nodes} as this would update the layout of the underlying treemap.

\subsection{Implementation}
The implementation of \tool{} mainly consists
of three parts, namely, VegaAR Editor, 
SpecHub, 
and AR viewers.
VegaAR Editor is a web-based application
that extends the Vega Editor~\cite{vegaEditor}, 
Vega Schema~\cite{vegaSchema} (\emph{i.e.}, for the \texttt{ar} block),
and Vega Compiler~\cite{vegaCompiler} (\emph{i.e.}, for the \feata{} and \featb{}).
SpecHub is a NodeJs-based application
that runs on a cloud server.
SpecHub also reuses the extended Vega Compiler in VegaAR Editor to parser
and generate \inlinefig{figures/icon_vv}.
We have implemented AR viewers based on Vuforia~\cite{vuforia}
on three different platforms,
including iOS (iPhone8 Plus), Android (Huawei P10), and web-based platform.
All AR viewers only provide minimal functionalities,
including QRCode decoder, 
AR image recognition,
and 3D registration.

==> tex/_deprecated/5-tool_bk.tex <==
\section{\tool{}}
\label{sec:tool}

This section introduces \tool{}, 
an authoring environment for augmented static visualizations \inlinefig{figures/icon_var}.
We first introduce its core workflow and then highlight its two bespoke features.
% by describing how do we design its core workflow
% and then enhance it with two advanced features step-by-step.

\subsection{Workflow}
% \cmo{The uniqueness of 
% AR extendable visualization
% lies in that it mixes
% the real and virtual visualization,
% which means the designer is required
% to create both 
% the reality (\emph{i.e.}, traditional 2D visualization to be printed on papers)
% and the virtuality (\emph{i.e.}, virtual visualization to be displayed in AR environments). Already use in intro}
% \ben{bit repetitive---should all be said in intro+relwork:}
% To create an AR extendable visualization,
% the designer is required to create both 
% the reality (\emph{i.e.}, the printed visualization)
% and the virtuality (\emph{i.e.}, the virtual visualization).
% On the one hand,
% the visualization community has developed
% many tools~\inlinefig{figures/icon_vis.png} 
% to help designers with various expertise
% create traditional 2D visualization.
% However, 
% these tools do not support creating virtual visualization that can be displayed in AR.
% \cmo{Revise/Remove this sentence} Moreover, it would be tedious and difficult for designers 
% to manually handle the technical details of AR systems.
% Thus, on the other hand,
% some researchers develop all-in-one
% tools~\inlinefig{figures/icon_vis+ar} (\emph{e.g.}, DxR~\cite{Sicat2019} and MARVisT~\cite{Chen2019}) 
% to support designers crafting visualizations in AR environments directly.
% However,
% these tools are not designed to create visualization for printing,
% and relative new \cmo{revise/remove this phase},
% limiting the designer to leverage the well-establish infrastructure libraries
% for creating 2D visualization.
% Thus, 
% solely using one kind of existing tools
% to create AR extendable visualization
% is strenuous.

\begin{figure}[thb]
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/workflow}
    \caption{A decoupled workflow creates both static and virtual visualizations.}
    \label{fig:workflow}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.99\columnwidth]{figures/pipeline}
    \caption{The main user interface and pipeline.}
    \label{fig:pipeline}
\end{figure*}

% To fulfil G1,
% the tool should be able to create both static \inlinefig{figures/icon_vr} 
% and virtual \inlinefig{figures/icon_vv} visualizations.
\tool{} creates both static \inlinefig{figures/icon_vr} 
and virtual \inlinefig{figures/icon_vv} visualizations.
Instead of developing a tool that combines both
the functionalities of visualization tools
for desktop \inlinefig{figures/icon_vis.png} and 
immersive \inlinefig{figures/icon_vis+ar.png} environments,
we abstract the common part of them
and propose a decoupled workflow (\autoref{fig:workflow}).
By separating the specification
(\emph{i.e.}, designing visualizations in \inlinefig{figures/icon_vis}) 
from the deployment
(\emph{i.e.}, presenting visualizations in \inlinefig{figures/icon_ar}),
our workflow allows designers without AR expertise 
to create both \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv}
in some well-established~\inlinefig{figures/icon_vis}
and leave the \inlinefig{figures/icon_ar} part to AR experts.

Specifically, 
our workflow adopts a browser/server architecture.
In the workflow, 
the designer uses a \inlinefig{figures/icon_vis}
to create a ``stem'' visualization~\inlinefig{figures/icon_v},
which then be captured as a \inlinefig{figures/icon_vr}.
While the \inlinefig{figures/icon_vr} is static,
the designer can continue updating \inlinefig{figures/icon_v},
similar to update a web page,
and use a converter~\inlinefig{figures/icon_converter} 
to convert it into a \inlinefig{figures/icon_vv}.
An AR viewer can be used to recognize the \inlinefig{figures/icon_vr}
and register the \inlinefig{figures/icon_vv}
to obtain the \inlinefig{figures/icon_var}.
By this mean, both \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv}
are created based on the same specification,
thus maintaining a high level of consistency.

We \cmo{implement} the workflow in \tool{} (\autoref{fig:pipeline})
by implementing its three components:
% which consists of three main components corresponding to the
\begin{itemize}
    \item \textbf{VegaAR Editor} is built based on Vega Editor~\cite{},
    a UI editor of Vega.
    Vega is a popular declarative grammar 
    for specifying data visualizations in JSON format,
    which strike a good balance between the simplicity and expressivity.
    In VegaAR Editor,
    the designer can create a \inlinefig{figures/icon_vr} 
    following the same practice in Vega
    and export the visualization as a static visualization (\autoref{fig:pipeline}c).
    Meanwhile, the designer can futher
    
    Meanwhile, different from the original Vega Editor,
    VegaAR Editor will generate a QRCode that contains the unique identity
    of the \inlinefig{figures/icon_vr} send its specification to a \textit{SpecHub}
    To augment the \inlinefig{figures/icon_vr} with one of the four augmentation methods,
    Then the designer can continue updating the specification of \inlinefig{figures/icon_vr},
    such as adding more data or defining multiple views.
    When satisfied with the updating,
    the designer can \texttt{publish} the updated specification to the \textit{SpecHub}.
    % All the modification after the exportation of the \inlinefig{figures/icon_vr}
    % will be link to the \inlinefig{figures/icon_vr} based on the QRCode and 
    % presented in AR as the \inlinefig{figures/icon_vv},
    % which means hitherto the designer does not need to explicitly specify AR and non-AR parts.
 
    % and generate a QRCode, 
    % which contains the meta information of the visualization (\emph{e.g.}, its unique identity and the web address of the \textit{Converter}), 
    % along with the visualization. 
    % \ben{it is not clear here how you extend Vega. what makes the the AR in vegaAR? what does the desginer has to do? Do they need to specify ar and non ar parts?}
    
    \item \textbf{SpecHub} is deployed on a cloud server 
    to receive and host the specifications from VegaAR Editor.
    Besides,
    it prepares all prerequisites for the \inlinefig{figures/icon_var},
    such as processing the specification of \inlinefig{figures/icon_vr} 
    to generate the AR reference image so that \inlinefig{figures/icon_vr} 
    can be recognized by AR viewers,
    differentiate the updated specification and the specification of \inlinefig{figures/icon_vr} to generate the \inlinefig{figures/icon_vv},
    hosting and returning the \inlinefig{figures/icon_vv} when it is fetched by AR viewers.
    
    \item \textbf{AR Viewer} is the endpoint (\emph{i.e.}, browser) 
    for audiences to view the \inlinefig{figures/icon_var}. 
    When scanning a \inlinefig{figures/icon_vr},
    an AR viewer will identify the \inlinefig{figures/icon_vv} based on its QRCode, 
    fetch its corresponding \inlinefig{figures/icon_vv} from the \textit{SpecHub},
    and register \inlinefig{figures/icon_vv} onto \inlinefig{figures/icon_vr}
    to present the \inlinefig{figures/icon_var} (\autoref{fig:pipeline}e).
    The AR viewer is not platform-specific.
    In this work, we have implement three AR viewers
    on the iOS, Android, and web-based platform, respectively.
\end{itemize}

With \tool{}, designers can easily create \inlinefig{figures/icon_var}
in one tool without digging into the AR details.

\subsection{Preview}
However,
a drawback of \tool{} is that it requires
the frequently switching between devices.
Indeed, it is challenging to
reconcile the conflict between 
designing on desktop platforms
and consuming on AR devices.
According to G2,
we can preview \inlinefig{figures/icon_vv} to alleviate this burden.
% However, 
% in terms of augmented static visualization, % \inlinefig{figures/icon_var},
% a method to alleviate this conflict
% is to simulate the AR scenario
% by previewing the \inlinefig{figures/icon_vv} and \inlinefig{figures/icon_vr} (G2),
% since \inlinefig{figures/icon_vr} will be part of the reality.
Besides, another glitch of \tool{} until now is that 
the designer cannot explicitly specify the \inlinefig{figures/icon_vv} 
in the specification.
We achieve G2 and fix the glitch together by introducing an advanced feature, \feata{}.

Specifically,
to preview the \inlinefig{figures/icon_vv} together with \inlinefig{figures/icon_vr},
the designer must explicitly specify how the \inlinefig{figures/icon_vv} is
during designing \inlinefig{figures/icon_vr},
which is not supported by the current Vega grammar.
Thus, we extend the Vega grammar
by adding an additional configuration block \texttt{ar} (\autoref{fig:pipeline}a) to it.
The \texttt{ar} block is optional in a specification
and will not affect the \inlinefig{figures/icon_vr}.
In the \texttt{ar} block,
the designer explicitly specify the augmentation method,
the visual encoding,
and the data of a \inlinefig{figures/icon_vv},
no matter the data is certain or uncertain:
\begin{itemize}
    \item \textbf{Certain}. 
    When the data is known,
    the designer can specify the \inlinefig{figures/icon_vv} 
    in the \texttt{ar} block,
    starting from define how it will augment \inlinefig{figures/icon_vr} in one of the four augmentation methods:
    1) in \textit{Extended View},
    the designer only need to specify 
    which datasets of \inlinefig{figures/icon_vr} will be appended with what data
    and reuse other visual encodings of the \inlinefig{figures/icon_vr};
    % , rather than specifying the visual encoding of \inlinefig{figures/icon_vv};
    2) in \textit{Composite View}, 
    % in addition to appending data to the detests of \inlinefig{figures/icon_vr}, 
    the designer can recursively specify a new visualization in the \texttt{ar} block
    with new datasets or the existing datasets of \inlinefig{figures/icon_vr};
    3) in \textit{Small Multiple},
    the designer only need to specify the new datasets and the layout of the virtual small multiples in relation to the \inlinefig{figures/icon_vr};
    4) in \textit{Multiple View}, the designer is allowed to create a complete new visualization in the \texttt{ar} block 
    and define its placement with respect to the \inlinefig{figures/icon_vr}.
    VegaAR Editor will preview the \inlinefig{figures/icon_vr} 
    with the \inlinefig{figures/icon_vv} (\emph{e.g.}, \autoref{fig:pipeline}b).
    % before publishing the visualization to be printed \cmo{GIVE a term to name this thing}.
    % Based on our study of the design space,
    % the designer can augment the printed visualization
    % with either new data or new visualization
    % in four different ways. 
    % Thus, in the \texttt{ar} block,
    % the designer can specify
    % the augmentation method
    % and then the augmentation details.
    % For example,
    % in~\autoref{fig:pipeline}a,
    % the designer specify that
    % the printed visualization will only be augmented with more data (\emph{i.e.}, the first augmentation method in the design space \cmo{GIVE names for the four augmentation methods})
    % and the additional data will be appended to the \texttt{``tree''}
    % dataset of the original specification.

    % If the designer choose other augmentation methods,
    % in the \texttt{ar} block
    % he can recursively define 
    % the new visualization with its specification,
    % which will also be previewed by \textit{VegaAR Editor}.

    \item \textbf{Uncertain}.
    The data of the \inlinefig{figures/icon_vv} could be uncertain during the creation 
    (\emph{e.g.}, the data can only be obtained in the future).
    In this case,
    it will be arduous for the designer to image the \inlinefig{figures/icon_vv}.
    We provide a \texttt{placeholder} mechanism to
    allow designers generate mockup data using wildcard~\cite{}.
    In the \texttt{ar} block, 
    the designer can create placeholder datasets
    and generate their data by 
    specifying the data type (\emph{e.g.}, categorical, temporal, and quantitative),
    number of datum,
    and ranges or potential options of the values
    of each column.
    VegaAR Editor will preview the placeholder datasets of \inlinefig{figures/icon_vv}.
    % to facilitate the design.
\end{itemize}

By explicitly define the \inlinefig{figures/icon_vv} in the \texttt{ar} block,
VegaAR Editor can preview the virtual content and simulate the AR scenario
on the desktop platform, %helping the designers
reducing the switching between devices.

\subsection{Auto-Hint}
%% motivation
% Our design space is built upon the validness model 
% that requires 
% the designer to ensure the AR visualization is valid
% In the design space,
% three augmentation methods can guarantee 
% the visualization is valid
% while the remaining one (\emph{i.e.}, 
% when augmenting the same visualization with more data.
% requires the designer to check the validity of the AR visualization.

\textit{Extended View} can easily be invalid
given the data dependency between \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} (\emph{e.g.}, the pie chart in Sec.\ref{ssec:model} and the tree diagram in Sec.\ref{sec:usage-scenario}).
In practice,
a visualization can be more complex by involving several datasets and visualization diagrams.
Thus, when choosing this augmentation methods,
the authoring environment should feature automatically method
to assist the designer in verifying the validity of the design
and provide hints for debugging invalid visual encodings (G3).

% automatic method is required to assist
% designers in verifying the validity of the AR visualization
% and fixing the visualization if it is invalid.

% However, it would be difficult to manually
% check the validity of the AR visualization,
% especially
% when its data or visual encoding are complex.
%% challenge
% For instance,
% for a hierarchical dataset,
% if new data will be added to its internal nodes,
% it cannot be visualized using a treemap
% but a node-link tree,
% since the layout of the treemap will be rearranged.
% However,
% if the internal nodes to be appended with new children 
% are not the deepest,
% the hierarchical dataset cannot be visualized as a node-link tree 
% using the ``cluster'' method~\cite{}; 
% instead, the ``tidy'' method~\cite{} could be used.


\begin{figure}[thb]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/dataflow}
    \caption{Auto-hint based on the comparison of the dataflow.}
    \label{fig:dataflow}
\end{figure}

%% solution
Instead of using a rule-based method,
we propose to validate the visualization
by comparing the dataflow between \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_var}.
%% the process of visualization
A general visualization process of a dataset $D_r$
can be summarize in~\autoref{fig:dataflow}:
$D_r$ will first be processed by
a serials of data transforms
and then mapped to visual channels
to construct the \inlinefig{figures/icon_vr}.
%% when will be valid
As demonstrated in Sec.\ref{ssec:augmentations},
in a valid \inlinefig{figures/icon_var},
the \inlinefig{figures/icon_vr} should remain unchanged
after appending the new data $D_v$,
which means the intermediate state $D_r^{Tn}$
before the visual mapping 
should also be unchanged.
Thus,
for each data transform,
we can compare 
the intermediate state of $D_r$ between the \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_var}
to see whether the intermediate state is the same.
If a intermediate state is changed,
for example ${D'}_r^{T2} \neq D_r^{T2}$,
it means the transform (\emph{i.e.}, Transform$2$)
makes the \inlinefig{figures/icon_vr} changed after appending new data,
thus leading to an invalid \inlinefig{figures/icon_var}.
Thus, 
we can give the designer 
a hint specific to the transform 
and further provide messages for fixing it (\emph{e.g.}, \autoref{fig:dataflow}a)
regardless of the complexity of the visualization.
% In practic, 
% only the data attributes that have been encoded by visual channels will be checked.

\subsection{Implementation}
The implementation of \tool{} mainly consists
of three parts, namely, VegaAR Editor, 
Converter, 
and AR Viewers.
VegaAR Editor is a web-based application
that extends the Vega Editor~\cite{}, 
Vega Schema~\cite{},
and Vega Compiler~\cite{}.
Converter is a NodeJs-based application
that runs on a cloud server.
Converter also reused the extended Vega Compiler
in VegaAR Editor to parser
and generate new virtual visualization based on new data.
To verify the cross platform capability of our approach,
we have implemented AR Viewers on three different platforms,
including iOS, Android, and web-based platform.
All AR Viewers only provide minimal functionalities,
including QRCode decoder, 
AR image recognition,
and 3D registration.

==> tex/_deprecated/5.5-examples.tex <==

\begin{figure*}[h!]
    \centering
    \includegraphics[width=2.1\columnwidth]{figures/example2}
    \caption{Examples created by \tool{}. \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv} indicate the static and virtual visualization, respectively.
    }
    \label{fig:gallery}
\end{figure*}

\section{Examples and Scenarios}

\autoref{fig:outdated-tl} and \autoref{fig:gallery}
present examples varying in
data type,
chart type,
augmentation method,
media,
and purpose.
We summarize scenarios that can benefit from augmenting static visualizations \inlinefig{figures/icon_var}.

%% extend canvas
\textbf{Overcoming space limitations}---AR can extend a static visualization where the space is scarce.
For example, 
in \autoref{fig:outdated-tl}a, 
given that much space of the newspaper is occupied by the banner,
the data journalism uses a \inlinefig{figures/icon_var}
to extend the canvas for visualization, thereby presenting additional data.
A similar usage can be found in the example of poster (\autoref{fig:gallery}a),
leaflet (\autoref{fig:gallery}f), name card (\autoref{fig:gallery}i),
and resume (\autoref{fig:gallery}j).
Moreover, 
in the wall-sized timeline in \autoref{fig:outdated-tl}b,
it is difficult to physically extend the wall for presenting updated data.
By using \inlinefig{figures/icon_var}, the designer can easily break through the limitation of physical world and present more information.

\textbf{Displaying new data}---AR can update the static visualizations,
thus providing the latest information 
and saving the cost to recreate them.
In real world,
information is can be updated frequently
while the materials to present the information might not.
\inlinefig{figures/icon_var} is a promising way to relieve
the mismatch between the update cycle of materials and information.
\autoref{fig:outdated-tl}b presents a representative example of using AR
to update a wall-sized timeline, which has been outdated for more than three years.
\autoref{fig:gallery}g demonstrates 
a stock market book
uses \inlinefig{figures/icon_var} 
to provide the latest S\&P index data
to help the reader better understand the historical context.
Generally users can also use \inlinefig{figures/icon_var}
to keep their information in static visualizations online.
For example, \autoref{fig:gallery}i is an academic name card
with google scholar citations that will not be outdated after distributing.

\textbf{Showing details}---AR can empower static visualizations with the capability to show details on demand.
``Overview first, zoom and filter, then details on demand''~\cite{Shneiderman1996}
is a well-known information visualization guideline
yet can hardly be followed in static visualizations.
\inlinefig{figures/icon_var} can achieve this classic visualization technique on static visualizations.
For example, \autoref{fig:gallery}a presents 
the overview hierarchical architecture of a university
and collapses the detail nodes into AR, thus avoiding information overload. 
As shown in \autoref{fig:gallery}h and j, many tree diagrams can benefit from this feature.

\textbf{Complementing additional data}---Visualizations in public spaces,
\inlinefig{figures/icon_var} 
can be used to overlay personal data.
For example,
in \autoref{fig:outdated-tl}c,
by overlaying the trajectories data onto a public map, 
\inlinefig{figures/icon_var} complements the geographical visualization with the user's own data, thus helping the user to understand his/her movement pattern.
Another example of complementing visualizations is
to provide supplemental information.
The leaflet advertisement in \autoref{fig:gallery}f
shows the salaries of other departments in AR for comparison purpose,
since this extra information is not the focus of the advertisement 
but can help readers obtain the context information.

\textbf{Protecting privacy}---\inlinefig{figures/icon_var} 
can protect individuals privacy. In \autoref{fig:gallery}e, the teacher printed the class' summary statistics for an exam, overlaying a student's personal ranking in \inlinefig{figures/icon_var}.
Similarly, \autoref{fig:gallery}h shows a projected chart for the new students to check their private information.


% In the example XX, teacher printed the statistic of questions of an exam in the paper checking section. 
% % To avoid students seeing others' scores, teachers created extendable boxplots with their own scores shown under AR environment using \tool
% The expressiveness of \tool{}
% is rooted in the visualization toolkit that it extends, \emph{i.e.}, Vega.
% Thus \tool{} supports a wide range of \textbf{charts} for various \textbf{data types}.
% For example, \autoref{fig:gallery}a and j 
% present tree diagrams of hierarchical data
% that can be augmented with more child or parent nodes.
% \autoref{fig:outdated-tl}c and \autoref{fig:gallery}g are two geographical visualizations
% that can be augmented with spatial-temporal data.
% Besides, the designer can easily achieve the four \textbf{augmentation methods}
% using the \texttt{ar} block, including 
% \textit{Extended View} (\autoref{fig:gallery}a, b, c, and d), 
% \textit{Composite View} (\autoref{fig:outdated-tl}c and \autoref{fig:gallery}e),
% \textit{Small Multiple} (\autoref{fig:gallery}f), 
% and \textit{Multiple View} (\autoref{fig:gallery}g).
% %% what's more
% Moreover, 
% \tool{} allows exciting \textbf{purposes} 
% by augmenting static visualizations in different \textbf{media}.
% For instance, 
% data journalism can reveal the supplemental data in AR (\emph{i.e.}, show more)
% in case the space of the newspaper is limited (\autoref{fig:outdated-tl}a).
% Designers can use AR to present the updated information (\emph{i.e.}, show new) 
% without recreating the whole product,
% saving much cost (\emph{e.g.} the wall-sized visualization in \autoref{fig:outdated-tl}b and the book in \autoref{fig:gallery}g).
% It is also possible to present personal data (\emph{i.e.}, show personal)
% in a public context (\emph{e.g.}, projections) for each individual 
% to protect privacy (\autoref{fig:gallery}e) 
% or support customization (\autoref{fig:gallery}h).
% Last but not least, besides presenting information,
% augmented visualizations can be used as creative products 
% for self-promotion (\autoref{fig:gallery}i, j) and even for gifting.
% \ben{I need to think how to introduce more structure in this section. Its very much a list but it's hard to get the message. are there types of scenarios, e.g.: 'adding new data', 'correcing data', 'complememnting'... ?}

% A range of AR printed visualizations can be built with various type of datasets and paper media using \tool. Table XX shows a summary of all examples. These examples can be found in XXX.

% \subsection{Various type of datasets}
% Tabular data can be used to build AR printed visualization using \tool. 
% Simple charts e.g. bar charts, boxplots, line charts, area charts, can be created. 
% Without \tool, designers need to create extra new infographics whenever new data come. Moreover, designers would involve in writing problems for AR viewers. 
% Finally, designer could easily create visualizations violating the AR printed visualization design space as mention in section XX. 
% With \tool, designers could easily create valid AR printed visualization. 
% %% paper checking
% % In the example XX, teacher printed the statistic of questions of an exam in the paper checking section. 
% % To avoid students seeing others' scores, teachers created extendable boxplots with their own scores shown under AR environment using \tool.

% Spatial-temporal and hierarchical data often required large spaces. 
% Temporal data also requires frequent updates. These characteristics provide opportunity for AR technology. 
% %% MAP
% In example XX, geo-trajectory data are shown in AR on the map. 
% In example XX, more children nodes can be observed under AR viewer.

% \subsection{Various type of paper media}
% Some infographics are put on newspapers, leaflets and books to give readers intuitive insight. 
% However, due to limited space on the physical media, large infographics are seldom used. With \tool, designer can control the number of data to be shown on newspapers to reduce the size of the article infographics. 
% The remaining data can be viewed under AR environment. 
% In example XX, the author? of the newspaper decided to print the infographics with data that are not mention in the paragraph. 
% In example XX, the author of the leaflet presented some additional information (i.e. comparisons) under AR viewers. 
% Viewers have no problem if they ignore the information under AR viewers. 
% In example XX, the book provided AR printed charts to show the up to date statistics for students.


% Large infographics are often printed on posters. 
% Created such visualization required some resources and time. 
% It takes much more resources to use electronic poster. 
% Therefore, AR technology can be a solution on this. 
% AR printed poster could be updated without any resources and time. 
% In the example XX, the AR visualization updated when the designer updated the data.

% To impress the employers in the first glance, employees might put some infographics on their CVs or name cards. 
% It is not good to show out of date data. 
% In the example X, the bar chart on the name card remains up to date under AR viewers. 
% In the example XX, the employee shows the hierarchical structure of his skills under AR viewer.


==> tex/_deprecated/6-evaluations_bk.tex <==
\newpage
\section{User Study}
We conducted a controlled user study to assess usability and utility of \tool{}. 
The study evaluated whether visualization designers
can create augmented static visualizations using \tool{}, 
evaluating the tool's usefulness and its two advanced features, 
\emph{i.e.}, \feata{} and \featb{}.

\subsection{Experimental Setting}

\newcommand{\base}{\textsc{Base}}
\newcommand{\pro}{\textsc{Pro}}

\textbf{Baseline technique:}
We provided a \textit{base mode} (\base{}) and a \textit{pro mode} (\pro{}) of \tool{}.
\pro{} provides full features of our authoring environment
while the \base{} does not provide the \feata{} and \featb{}.
To control the study length,
we also provide the \texttt{ar} block (without the visual preview) 
in \base{} for designers to explicitly define the virtual visualization.

% \ben{this below section is a bit confusing---I suggest structuring it by tasks: T1: say everything about T1, T2: .. remember that reviewers want to look back to understand that these tasks were.}
\textbf{Tasks:}
Different from other authoring systems~\cite{},
our system allows users to create visualizations with new forms (\emph{i.e.}, static plus augmented) in a ``traditional'' way (\emph{i.e.}, Vega).
Thus, we design a controlled free-form study rather than a reproduction study~\cite{}.
Specifically,
to simulate a concrete scenario related to the campus where the participants were recruited,
we took the poster example in \autoref{fig:gallery}k (without AR visualizations)
and asked study participants to complete the poster
by creating the four visualizations 
(referred to as tasks T1 - T4). 
T1-T4 cover a wide range of data types
and extend the visualization as an \textit{Extended View}--- 
the most challenging augmentation method (Sec.\ref{sec:design_space}).
For each task,
participants were provided with
the background information,
relevant Vega documents,
a instruction to load the dataset.
% and two Vega examples as the starting point.
% In each task,
% the participants were required to visualize a part of it in reality and the remaining part in virtuality. 
% Besides, each task further provides: % 
The detail configurations of each tasks are as follows:
% and \textit{2)} two Vega examples as starting point.
% To control the study focus, we further configured the tasks as follows:

\begin{enumerate}[label={\textbf{T\arabic*}}, leftmargin=*]
    \item provided a hierarchical dataset about the university structure
    and two Vega examples, \emph{i.e.}, a node-link tree and a treemap example.
    The treemap was ensured to be invalid for the dataset
    while the node-link tree was invalid in default but can be corrected to be valid by modifying one visual encoding.
    The purpose of this setting is to assess whether the participant can debug the invalid design in different mode.
    
%     Among the two provided Vega examples, only one 
%     suitable for the poster context while the aspect ratio of 
% (\emph{e.g.}, the ratio of another example cannot fit into the poster),

    \item had the same purpose as \textbf{T1} and provided a network dataset about the collaboration among faculties in CSE and two Vega examples, \emph{i.e.}, a matrix diagram and a radial node-link graph.
    The radial node-link graph was ensured to be invalid for the dataset
    while the matrix diagrams was invalid in default 
    but can be corrected to be valid by modifying one visual encoding.
    
    \item provided a temporal dataset about the mean in-lab time of the PG students in CSE and two examples, \emph{i.e.}, a single line chart and a multiple line chart.
    Both two examples can be valid without any corrections.
    We deliberately put the text description of \textbf{T3} on the right 
    to see how the participants deal with the potential occlusions due to the AR extension
    in different mode.

% for T1, T2,
% only one example is suitable for the poster context
% (\emph{e.g.}, the ratio of another example cannot fit into the poster),
% each of which contains one and only one 
% inappropriate visual encoding leading to an invalid augmented visualization \ben{no sure I understand that previous sentence}.
% makes the example 
% invalid for the provided data 
% (\emph{e.g.}, the ``cluster'' layout method mentioned in Sec.\ref{sec:usage-scenario}).
% The main purpose is to assess whether the participant 
% can manually debug the inappropriate visual encoding \ben{what are you providing them with?}. 

    \item provided a geographic dataset about the campus checking data of PG students in CSE
    and a contour map example.
    The example was invalid in default for the dataset but can be corrected to be valid by modifying one visual encoding. 
    However, the default invalid design will only lead to a unnoticeable mismatch (but can be detected by our \featb{}) between the real and virtual visualizations.
    By this, besides the same purposes of \textbf{T1} and \textbf{T2},
    we further want to see how the participants handle the conflict 
    between their observation and our hints.
\end{enumerate}
The materials we provided to the participants can be found in the supplemental materials.

\textbf{Participants and Apparatus:}
We recruited 12 participants (8 male; age range: 22-30, average 25.6),
who had at least two years experience with D3 or Vega (since Vega is built based on D3)
and no expertise in AR programming (\emph{e.g.}, Unity).
% The candidates with more experiences on Vega had a higher priority to be invited.
According to the pre-study survey,
all participants had more than two years experience on data visualization ($\mu = 3.54, \sigma = 1.44$).
% For expertise on using visualization tools,
% participants reported 5 ``Expert'' and 7 ``Knowledgeable'' on D3,
% while 5 ``Knowledgeable' and 7 ``Novice'' on Vega.
% We considered all the participants can 
% independently create visualizations
% based on the examples of Vega with minimal guidance.
% They were also not the co-authors of the paper. 
% The participants were identified as P1-P12, respectively. 
Each participant received a gift card worth \$14 
at the beginning of the session, independent of their performance. 
The study was run in the lab, using a 15-inch laptop, or their own their own. 
A 5.5-inch mobile AR viewer was provided to view the AR visualization \ben{what AR viewer is this?}.

\begin{figure}[th]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/userstudy_protocol.png}
    \caption{Participants completed four tasks, two in each of two conditions (\base or \pro). The conditions were counter-balanced across participants, thus each participant completing only one path in this figure.}
    \label{fig:userstudy-protocol}
\end{figure}

\textbf{Procedure:}
Our within-subject study design followed 6 stages, summarized in Figure \ref{fig:userstudy-protocol}.
%% introduce augmented visualization Vega and
We first introduced the purpose of the study,
explained the concept of valid augmented visualizations
via examples (\emph{i.e.}, an augmented bar chart and an augmented pie chart\ben{, see Section XX}), introduced Vega, as well as how to create a visualiation with \tool{} 
\ben{how long did you explain them stuff?} (\textit{introduction}).
Participants then were given a step-by-step \textit{training} instruction 
about reproducing the two aforementioned examples 
and asked to reproduce them 
\ben{be specific about the examples (e.g., figures). How long did you give them to do it?}.
Participants were encouraged to ask questions and explore other examples with our system \ben{again, say how long you gave them to play around}.

\ben{I don't understand the differences between groups. can you explain in fig.7?} 
We performed a within-subject study on T1-T4,
two in each of two conditions: \base{} and \pro. The \pro-group started with the \pro-condition and then performed on \base, the \base-group did start with \base-condition. The four tasks were divided into two groups (T1\&T3 \emph{vs}. T2\&T4) to balance the workload across \base{} and \pro{} \ben{is this previous correctly said?}. 
Before performing with \pro, participants were given an instruction sheet with an explanation of the advanced features (\ben{name features here})
and were encouraged 
to explore the pro version and ask questions.
To avoid information overload,
we provided participants with the resource package of a task
after finishing the previous task\ben{What is a resource-package?}.
Participants were encouraged to explore, ask question about, 
and get familiar with the resources before each task \ben{again exploration?}.
A task was started 
when a participant was confident and confirmed to begin
and ended when the participants confirmed finishing.
We counterbalanced the order of the conditions and groups of tasks across participants. 

At the end, participants completed a post-study questionnaire
and answered a few questions of a semi-structured interview
to collect subjective feedback.
In total, each study session lasted approximately 1.5-2 hours.
The experimental protocol is shown in~\autoref{fig:userstudy-protocol}.

\ben{I created shortcuts for these measures( italic in brackets), which you can reuse in the analysis.  Do you have objective criteria how you measure (record) and assess them? If so, name them here. It feels like this would be something sensitive to have since your measures are not easy to quantify. A picky reviewer might object here and question your study.}
\textbf{Task Performance Measures:}
For each task we recorded task completion \textit{time} and \textit{correctness} of each task.
A correct design should
1) fit the poster context \ben{(\textit{fit})}, 
2) does not occlude its text description \ben{(\textit{clutterfree})},
and 3) follows our valid model \ben{(\textit{validity})}.
All measures are explicitly explained to the participants before the tasks.

%%%%%%%%%%%%%%%%


\subsection{Time and correctness}

\begin{figure}[th]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/user-study0.pdf}
    \caption{Left: Average task completion time and 98\% CIs across tasks. Right: The correct rate across tasks.}
    \label{fig:quant-results}
\end{figure}

\ben{why 98\%CIs. if you show .98, then you need to report on p<.02.}
\ben{Results are summarized in Figure \ref{fig:quant-results} showig 98\% confidence intervalls (CIs).} Significance values are reported for $p <.05 (\ast)$, $p <.01 (\ast\ast)$, and
$p <.001 (\ast\ast\ast)$, abbreviated by the number of stars. % in parenthesis.

\textbf{Completion Time:}
As expected \ben{this requires some hypotheses. you can mention them above}, 
participants finished the tasks faster with \pro{} ($\mu=278s$, $98 \%CI = [206, 351]$)
than with \base{} ($\mu = 557s$, $98 \%CI = [413, 701]$).
% Average finish times are 278$s$ for pro mode ()
% and 557$s$ for base mode ().
Before more detailed probes \ben{probes?}, 
we first confirmed that all results of completion times in each condition
follow normal distribution using Anderson-Darling test.
Using an independent-samples t-test with a null hypothesis that
the participants perform equally fast in each mode,
we found that participants performed significantly
faster \pro{} on T1 ($\ast\ast$), T2 ($\ast$), and T3 ($\ast\ast$). No significant difference was observed for completion time
on T4 ($p = 0.14$).

\textbf{\ben{Correctness}:}
As for the correctness,
almost all of the augmented visualizations (23/24) created in \pro{} were correct \ben{again, how did you quantify that?}
while only a few \ben{more than 1/3 is not few} correct augmented visualizations (9/24) were created 
without the help of \feata{} and \featb{}.
Given the correctness follows Bernoulli distribution \ben{how did you quantify that? is correctness a continuous value, e.g., between 0 and 1?},
we used Binomial Test with a null hypothesis 
that the result has a equal chance to be correct or wrong,
by which significant positive effects were observed
on T2-T4 ($\ast$) in \pro and 
no significant effect was observed in other cases.

% We repeated t-test on the validness of designs,
% by which significant effects were observed
% on T1 ($p < .01$), T2 ($p < .05$), and T4 ($p < .05$).
% A marginally significant difference was observed for validness on T3 ($p = 0.09$).

\begin{figure}[th]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/user-study1.pdf}
    \caption{Means and 98\% CIs of post-study self-reported efficiency, effectiveness, and mental demand on a scale from 1 (more on base mode) to 7 (more on pro mode).}
    \label{fig:self-report}
\end{figure}

\textbf{Post-Study Feedback:}
Anderson-Darling test reveals that the post-study self-reported results
did not follow normal distribution. 
Thus, we used a one-sample non-parametric Wilcoxon signed rank test 
with a null hypothesis that the result is middle Likert scale value. % (\emph{i.e.}, 4). 
We found significant positive effects for participants' self-reported efficiency in ($\ast\ast\ast$) and effectiveness ($\ast\ast$) \pro{}. For \base,
a significant negative effect was observed for
the participants' self-reported mental demand ($\ast\ast$) (Figure \ref{fig:self-report}).
\ben{explain high-level findings from Figure \ref{fig:subjective}} 
%Qualitative feedback is summarized \emph{w.r.t} the usability of the system, and usefulness and satisfaction of the two features.

\begin{figure}[th]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/user-study2.pdf}
    \caption{Subjective feedback on the usability of the authoring environment, usefulness and satisfaction of the two features, including means and 98\% CIs. Distributions of the rating are shown on the left.}
    \label{fig:subjective}
\end{figure}

\textbf{Usability:}
Targeting general visualization designers
is kept in our mind during designing our authoring environment.
Overall the participants spoke highly of the usability
of our system as it is \textit{easy to learn} ($\mu=6.50, 98\% CI = [6.05, 6.95]$) and \textit{easy to use} ($\mu=6.33, 98\% CI = [5.90, 6.77]$).
With our system, all the participants without AR expertise
could successfully create augmented visualizations in a short time.
We observed that most of the participants felt excited when they
viewed their creations through the AR viewer.
P8 commented that \textit{``I have never tried Unity and AR things''} but our system \textit{``can help us quickly produce AR extensible visualizations.''}
When we asked the participants 
whether they want more control of the AR details
(\emph{e.g.}, fancy visual effects),
all participants thought 
that the tool should be cost-effective 
and remain simple \textit{``unless coding the AR details are necessary for the task.''}

\textbf{Usefulness.}
When considering the two features of our authoring environment,
the participants commented positively and confirmed
the usefulness of \feata{} ($\mu=6.92, 98\% CI = [6.72, 7.11]$)
and \featb{} ($\mu=6.50, 98\% CI = [6.05, 6.95]$).
Although we provided an AR viewer for participants
to check their design in the study,
participants didn't use it frequently since
\textit{``\feata{} is enough thus no need to switch to the AR device''} (P2)
and \textit{``it provides immediate feedback.''} (P9).
Participants also agreed the usefulness of \featb{}.
As pointed out by P4,
who had 6 years experiences on data visualizations,
\textit{``the \featb{} is really important for the debug''}.
Indeed, the participants were able to finish
the creation more quickly and effectively with these two features,
just like P10 noted that \textit{``creation process is tedious without \featb{} and \feata{}.''}

\textbf{Satisfaction:}
The participants also responded high user satisfactions of
the design of \feata{} ($\mu=6.75, 98\% CI = [6.45, 7.05]$)
and \featb{} ($\mu=6.67, 98\% CI = [6.23, 7.10]$). 
Participants expressed that \feata{} was \textit{``intuitive''} (P12) and \textit{``quiet'' }(P6),
but \textit{``has done all it should do.''} (P6)
As for \featb{},
P6 suggested us to \textit{``highlight this feature in your paper''};
otherwise \textit{``you will undersell it.''}
Others' comments also indicated improvements of \featb{},
including \textit{``better highlight the problematic code''} (P2)
and \textit{``improve the error descriptions.''} (P7)

\subsection{Observation and Discussion}
Creating augmented visualizations yields a different experience 
from creating desktop and immersive visualizations.
This section discusses observations and insights from our study.

\textbf{Whose faults? AR or my design?}
As discussed in Sec.~\ref{ssec:model},
inappropriate visual encoding may lead to a
mismatch between the static and virtual visualization.
During the study, we observed 
that some participants suspected the correctness of the AR viewer
and our implementation of AR at the first time
when there was a mismatch happened.
Even after confirming with us that there was nothing wrong with the AR part, 
some participants still doubted that the AR devices worked properly,
especially when designing without the help of \featb{}.
In practices, 
given that the AR details are similar to a ``black box'' in our workflow,
it is important to help designers distinguish the error from AR
and their designs in a trustworthy way.

\textbf{Where am I? Reality or virtuality?}
Creating augmented visualizations requires the designer
to maintain two designs in mind -- one for the reality and the other for the virtuality.
Although our system provide \feata{} to alleviate this burden,
we observed that sometimes participants were in disorder during the tasks.
For example,
some designers chose a line chart to present the temporal data in T3.
When they discovered that the 
augmented line chart would occlude the text description,
% which was put on the right of the poster deliberately,
they attempted to flip the chart to a right-to-left orientation
and stuck in the counter-intuitive design.
An interesting fact was that 
all the participants 
who stuck in T3 had more than 3 years experiences on visualization
while those with less than 3 years experiences directly
chose the multiple line chart.
We suspected this was due to their linear mindset for temporal data.
How to design more effective method to help designer close the gap between
the reality and virtuality during creaton is an important direction for future improvement.

\textbf{What is the hint? Ignore or follow?}
In pro mode, our authoring environment provides useful hints 
for debugging augmented static visualizations.
In the study, we observed that one participant ignore the hints
and attempted to correct the wrong design by himself 
(the only one who failed in T1 in the pro mode).
In the interview, he said ``I thought the hints are useless so I didn't read it.''
By contrast, most of the participants followed the hint but
admitted that they actually did not know what was wrong with their design.
However, the hint occasionally confuse the participants, \emph{e.g.}, in T4.
For the \textbf{contour} in the provided Vega examples for T4, 
the new data to be displayed in AR would 
lead to a unnoticeable mismatch % (which was also by design) 
between the reality and virtuality.
This mismatch could hardly perceived by human, but could be detected by our \featb{}.
Thus, the participants usually confused by the warning message 
and spent relative long time on T4, 
which we believe was the reason of no significant difference between base and pro mode was observed on T4.
We discussed this issue with the participants.
11 out of 12 participants agreed that the hints from \featb{} 
can be seemed as a ``strict mode warning'', 
which also supported our rationale to use it as warning instead of error.
In summary, although \featb{} is useful and satisfied by the participants,
it can be improved for more user-friendly and intelligence in the future.

==> tex/_deprecated/7-discussion.tex <==
\section{Future work and Limitations}

%We now reflect on broader issues and opportunities 
%that arose during our study 
%and acknowledge the limitations.

\textbf{Generalization to 3D and dynamic AR visualizations}---\tool{} currently focuses on 2D static \inlinefig{figures/icon_var} that goes beyond the desktop
but it can be generalized to 3D and dynamic \inlinefig{figures/icon_var}.
As has been proven successful in DXR~\cite{Sicat2019},
Vega grammar can be extended from 2D to 3D visualizations.
\tool{} also adopts and extends Vega grammar but in another direction, 
supporting the creation of both \inlinefig{figures/icon_vr} and \inlinefig{figures/icon_vv}.
It is possible to merge the extension and design from DXR,
thus allowing designers to create 3D \inlinefig{figures/icon_vv} in \tool{}.
Meanwhile, the Vega grammar inherently supports design interactive visualizations,
providing opportunities to bring interactivity and animation to \inlinefig{figures/icon_vr}.
%However, how to design valid 3D and dynamic \inlinefig{figures/icon_var} 
%demands further research as it may involve complex perception issues and design considerations.

\textbf{Multiple augmentations and multiple devices}--- % among multiple audiences.
Our design so far concentrates on augmenting one \inlinefig{figures/icon_vr} on one AR device.
A more challenging question is
how to design \inlinefig{figures/icon_var} that augment multiple \inlinefig{figures/icon_vr}
(\emph{e.g.}, the four visualizations on the poster in \autoref{fig:gallery}k) at once.
Besides, how to design \inlinefig{figures/icon_var} distributed 
% these multiple augmentations 
across multiple devices to support collaborations is also a challenging yet 
promising future direction.
%Once the \inlinefig{figures/icon_var} is interactive, the designer should further consider the cross devices interactions (\emph{e.g.}, HMDs prefer mid-air gestures and handheld devices use touch).

\textbf{Design with scene understandings}---%\inlinefig{figures/icon_var} closely integrate \inlinefig{figures/icon_vv}
% with the reality, which is primary the \inlinefig{figures/icon_vr} in this study.
In many real-world examples, the immediate environment influences readability and how a visualization is read. 
%can be more diverse and uncertain,
%which introduces both opportunities and challenges.
For example,
designers can create \inlinefig{figures/icon_vv} that 
adapts to the ambient light,
visualizes in-situ temperature data, % (\emph{e.g.}, the temperature data),
and or adapt more deeply to the AR-Canvas~\cite{bach2017drawing}. Recent progress in scene understandings of computer vision (CV)
offers possibilities to realize
such kind of environment adaptive visualizations.
% In the field of visualization,
% some researchers
% have explored employing these CV methods
% to understand the scene and aid the design
% (\emph{e.g.}, saliency detection~\cite{Bylinskii2017a} and style transfer~\cite{Chen2019b}).
% which cns leveraging these scene understanding methods
% to facilitate the design and presentation of \inlinefig{figures/icon_var}
% as an important future direction.

\textbf{Study Limitations}---Similar to other studies of authoring tools~\cite{Amini2017, Kim2019, Xia2018}, the sample size of our user study is small, given that access to experts is naturally limited. Further evaluation is thus suggested.
%We also used a within subject design 
% so the participants who saw the other version first may have more disappointment to the \base{}.
% Between group studies might affect the differences in confidence,
% but then preference cannot be collected. }
\tool{} currently generates a QRCode along with a \inlinefig{figures/icon_vr}
when publishing, which size and position can be configured in the \texttt{ar} block.
While the QRCode has a good usability and is a flag to attract audiences to scan, it adds a superfluous component to the visualization. Future study is required to optimize the QRCode
by striking a balance between functionality and aesthetics.

%% 3. tools? vega, generalize to other
%% 4. qr code physical specification

==> tex/_deprecated/_1-default.tex <==
\section{Page Size and Columns}
On each page your material should fit within a rectangle of 7 $\times$
9.15 inches (18 $\times$ 23.2 cm), centered on a US Letter page (8.5
$\times$ 11 inches), beginning 0.85 inches (1.9 cm) from the top of
the page, with a 0.3 inches (0.85 cm) space between two 3.35 inches
(8.4 cm) columns. Right margins should be justified, not
ragged. Please be sure your document and PDF are US letter and not A4.

\section{Typeset Text}
The styles contained in this document have been modified from the
default styles to reflect ACM formatting conventions. For example,
content paragraphs like this one are formatted using the Normal style.

\LaTeX\ sometimes will create overfull lines that extend into columns.
To attempt to combat this, the \texttt{.cls} file has a command,
\texttt{{\textbackslash}sloppy}, that essentially asks \LaTeX\ to
prefer underfull lines with extra whitespace.  For more details on
this, and info on how to control it more finely, check out
{\url{http://www.economics.utoronto.ca/osborne/latex/PMAKEUP.HTM}}.


\subsection{Title and Authors}

Your paper's title, authors and affiliations should run across the
full width of the page in a single column 17.8 cm (7 in.) wide.  The
title should be in Helvetica or Arial 18-point bold.  Authors' names
should be in Times New Roman or Times Roman 12-point bold, and
affiliations in 12-point regular.  

See \texttt{{\textbackslash}author} section of this template for
instructions on how to format the authors. For more than three
authors, you may have to place some address information in a footnote,
or in a named section at the end of your paper. Names may optionally
be placed in a single centered row instead of at the top of each
column. Leave one 10-point line of white space below the last line of
affiliations.

\subsection{Abstract and Keywords}

Every submission should begin with an abstract of about 150 words,
followed by a set of Author Keywords and ACM Classification
Keywords. The abstract and keywords should be placed in the left
column of the first page under the left half of the title. The
abstract should be a concise statement of the problem, approach, and
conclusions of the work described. It should clearly state the paper's
contribution to the field of HCI\@.

\subsection{Normal or Body Text}

Please use a 10-point Times New Roman or Times Roman font or, if this
is unavailable, another proportional font with serifs, as close as
possible in appearance to Times Roman 10-point. Other than Helvetica
or Arial headings, please use sans-serif or non-proportional fonts
only for special purposes, such as source code text.

\subsection{First Page Copyright Notice}
This template include a sample ACM copyright notice at the bottom of
page 1, column 1.  Upon acceptance, you will be provided with the
appropriate copyright statement and unique DOI string for publication.
Accepted papers will be distributed in the conference
publications. They will also be placed in the ACM Digital Library,
where they will remain accessible to thousands of researchers and
practitioners worldwide. See
\url{http://acm.org/publications/policies/copyright_policy} for the
ACM's copyright and permissions policy.

\subsection{Subsequent Pages}

On pages beyond the first, start at the top of the page and continue
in double-column format.  The two columns on the last page should be
of equal length.

\begin{figure}
\centering
  \includegraphics[width=0.9\columnwidth]{figures/sigchi-logo}
  \caption{Insert a caption below each figure. Do not alter the
    Caption style.  One-line captions should be centered; multi-line
    should be justified. }~\label{fig:figure1}
\end{figure}

\subsection{References and Citations}

Use a numbered list of references at the end of the article, ordered
alphabetically by last name of first author, and referenced by numbers
in
brackets~\cite{acm_categories,ethics,Klemmer:2002:WSC:503376.503378}.
Your references should be published materials accessible to the
public. Internal technical reports may be cited only if they are
easily accessible (i.e., you provide the address for obtaining the
report within your citation) and may be obtained by any reader for a
nominal fee. Proprietary information may not be cited. Private
communications should be acknowledged in the main text, not referenced
(e.g., ``[Borriello, personal communication]'').

References should be in ACM citation format:
\url{http://acm.org/publications/submissions/latex_style}. This
includes citations to internet
resources~\cite{acm_categories,cavender:writing,CHINOSAUR:venue,psy:gangnam}
according to ACM format, although it is often appropriate to include
URLs directly in the text, as above.


\begin{table}
  \centering
  \begin{tabular}{l r r r}
    % \toprule
    & & \multicolumn{2}{c}{\small{\textbf{Test Conditions}}} \\
    \cmidrule(r){3-4}
    {\small\textit{Name}}
    & {\small \textit{First}}
      & {\small \textit{Second}}
    & {\small \textit{Final}} \\
    \midrule
    Marsden & 223.0 & 44 & 432,321 \\
    Nass & 22.2 & 16 & 234,333 \\
    Borriello & 22.9 & 11 & 93,123 \\
    Karat & 34.9 & 2200 & 103,322 \\
    % \bottomrule
  \end{tabular}
  \caption{Table captions should be placed below the table. We
    recommend table lines be 1 point, 25\% black. Minimize use of
    table grid lines.}~\label{tab:table1}
\end{table}


\section{Sections}

The heading of a section should be in Helvetica or Arial 9-point bold,
all in capitals. Sections should \textit{not} be numbered.

\subsection{Subsections}

Headings of subsections should be in Helvetica or Arial 9-point bold
with initial letters capitalized.  For sub-sections and
sub-subsections, a word like \emph{the} or \emph{of} is not
capitalized unless it is the first word of the heading.

\subsubsection{Sub-subsections}

Headings for sub-subsections should be in Helvetica or Arial 9-point
italic with initial letters capitalized.  Standard
\texttt{{\textbackslash}section}, \texttt{{\textbackslash}subsection},
and \texttt{{\textbackslash}subsubsection} commands will work fine in
this template.


\section{Figures/Captions}

Place figures and tables at the top or bottom of the appropriate
column or columns, on the same page as the relevant text (see
Figure~\ref{fig:figure1}). A figure or table may extend across both
columns to a maximum width of 17.78 cm (7 in.).

\begin{figure*}
  \centering
  \includegraphics[width=1.75\columnwidth]{figures/map}
  \caption{In this image, the map maximizes use of space. You can make
    figures as wide as you need, up to a maximum of the full width of
    both columns. Note that \LaTeX\ tends to render large figures on a
    dedicated page. Image: \ccbynd~ayman on
    Flickr.}~\label{fig:figure2}
\end{figure*}

Captions should be Times New Roman or Times Roman 9-point bold.  They
should be numbered (e.g., ``Table~\ref{tab:table1}'' or
``Figure~\ref{fig:figure1}''), centered (if one line) otherwise justified, and placed beneath the figure
or table.  Please note that the words ``Figure'' and ``Table'' should
be spelled out (e.g., ``Figure'' rather than ``Fig.'') wherever they
occur. Figures, like Figure~\ref{fig:figure2}, may span columns and
all figures should also include alt text for improved accessibility.
Papers and notes may use color figures, which are included in the page
limit; the figures must be usable when printed in black-and-white in
the proceedings.

The paper may be accompanied by a short video figure (we recommend staying within five
minutes in length). However, the paper should stand on its own without
the video figure, as the video may not be available to everyone who
reads the paper.  

\subsection{Inserting Images}
When possible, include a vector formatted graphic (i.e. PDF or EPS).
When including bitmaps,  use an image editing tool to resize the image
at the appropriate printing resolution (usually 300 dpi).


\section{Quotations}
Quotations may be italicized when \textit{``placed inline''}.

\begin{quote}
Longer quotes, when placed in their own paragraph, need not be
italicized or in quotation marks when indented.  
\end{quote}

\section{Language, Style, and Content}

The written and spoken language of SIGCHI is English. Spelling and
punctuation may use any dialect of English (e.g., British, Canadian,
US, etc.) provided this is done consis- tently. Hyphenation is
optional. To ensure suitability for an international audience, please
pay attention to the following:

\begin{itemize}
\item Write in a straightforward style.
\item Try to avoid long or complex sentence structures.
\item Use common and basic vocabulary (e.g., use the word ``unusual'' rather than the word ``arcane''.
\item Briefly define or explain all technical terms that may be
  unfamiliar to readers.
\item Explain all acronyms the first time they are used in your
  text---e.g., ``Digital Signal Processing (DSP)''.
\item Explain local references (e.g., not everyone knows all city
  names in a particular country).
\item Explain ``insider'' comments. Ensure that your whole audience
  understands any reference whose meaning you do not describe (e.g.,
  do not assume that everyone has used a Macintosh or a particular
  application).
\item Explain colloquial language and puns. Understanding phrases like
  ``red herring'' may require a local knowledge of English.  Humor and
  irony are difficult to translate.
\item Use unambiguous forms for culturally localized concepts, such as
  times, dates, currencies, and numbers (e.g., ``1--5--97'' or
  ``5/1/97'' may mean 5 January or 1 May, and ``seven o'clock'' may
  mean 7:00 am or 19:00). For currencies, indicate equivalences:
  ``Participants were paid {\fontfamily{txr}\selectfont \textwon}
  25,000, or roughly US \$22.''
\item Be careful with the use of gender-specific pronouns (he, she)
  and other gendered words (chairman, manpower, man-months). Use
  inclusive language that is gender-neutral (e.g., she or he, they,
  s/he, chair, staff, staff-hours, person-years). See the
  \textit{Guidelines for Bias-Free Writing} for further advice and
  examples regarding gender and other personal
  attributes~\cite{Schwartz:1995:GBF}. Be particularly aware of
  considerations around writing about people with disabilities.
\item If possible, use the full (extended) alphabetic character set
  for names of persons, institutions, and places (e.g.,
  Gr{\o}nb{\ae}k, Lafreni\'ere, S\'anchez, Nguy{\~{\^{e}}}n,
  Universit{\"a}t, Wei{\ss}enbach, Z{\"u}llighoven, \r{A}rhus, etc.).
  These characters are already included in most versions and variants
  of Times, Helvetica, and Arial fonts.
\end{itemize}


\section{Accessibility}
The Executive Council of SIGCHI has committed to making SIGCHI
conferences more inclusive for researchers, practitioners, and
educators with disabilities. As a part of this goal, the all authors
are asked to work on improving the accessibility of their
submissions. Specifically, we encourage authors to carry out the
following five steps:
\begin{enumerate}
\item Add alternative text to all figures
\item Mark table headings
\item Add tags to the PDF
\item Verify the default language
\item Set the tab order to ``Use Document Structure''
\end{enumerate}
For more information and links to instructions and resources, please
see: \url{http://chi2016.acm.org/accessibility}.  The
\texttt{{\textbackslash}hyperref} package allows you to create well tagged PDF files,
please see the preamble of this template for an example.

\section{Page Numbering, Headers and Footers}
Your final submission should not contain footer or header information
at the top or bottom of each page. Specifically, your final submission
should not include page numbers. Initial submissions may include page
numbers, but these must be removed for camera-ready. Page numbers will
be added to the PDF when the proceedings are assembled.

\section{Producing and Testing PDF Files}

We recommend that you produce a PDF version of your submission well
before the final deadline.  Your PDF file must be ACM DL
Compliant. The requirements for an ACM Compliant PDF are available at:
{\url{http://www.scomminc.com/pp/acmsig/ACM-DL-pdfs-requirements.htm}}.

Test your PDF file by viewing or printing it with the same software we
will use when we receive it, Adobe Acrobat Reader Version 10. This is
widely available at no cost. Note that most
reviewers will use a North American/European version of Acrobat
reader, so please check your PDF accordingly.

\section{Conclusion}

It is important that you write for the SIGCHI audience. Please read
previous years' proceedings to understand the writing style and
conventions that successful authors have used. It is particularly
important that you state clearly what you have done, not merely what
you plan to do, and explain how your work is different from previously
published work, i.e., the unique contribution that your work makes to
the field. Please consider what the reader will learn from your
submission, and how they will find your work useful. If you write with
these questions in mind, your work is more likely to be successful,
both in being accepted into the conference, and in influencing the
work of our field.

\section{Acknowledgments}

Sample text: We thank all the volunteers, and all publications support
and staff, who wrote and provided helpful comments on previous
versions of this document. Authors 1, 2, and 3 gratefully acknowledge
the grant from NSF (\#1234--2012--ABC). \textit{This whole paragraph is
  just an example.}

  
% Use a numbered list of references at the end of the article, ordered
% alphabetically by first author, and referenced by numbers in
% brackets~\cite{ethics, Klemmer:2002:WSC:503376.503378,
%   Mather:2000:MUT, Zellweger:2001:FAO:504216.504224}. For papers from
% conference proceedings, include the title of the paper and an
% abbreviated name of the conference (e.g., for Interact 2003
% proceedings, use \textit{Proc. Interact 2003}). Do not include the
% location of the conference or the exact date; do include the page
% numbers if available. See the examples of citations at the end of this
% document. Within this template file, use the \texttt{References} style
% for the text of your citation.

% Your references should be published materials accessible to the
% public.  Internal technical reports may be cited only if they are
% easily accessible (i.e., you provide the address for obtaining the
% report within your citation) and may be obtained by any reader for a
% nominal fee.  Proprietary information may not be cited. Private
% communications should be acknowledged in the main text, not referenced
% (e.g., ``[Robertson, personal communication]'').


% Balancing columns in a ref list is a bit of a pain because you
% either use a hack like flushend or balance, or manually insert
% a column break.  http://www.tex.ac.uk/cgi-bin/texfaq2html?label=balance
% multicols doesn't work because we're already in two-column mode,
% and flushend isn't awesome, so I choose balance.  See this
% for more info: http://cs.brown.edu/system/software/latex/doc/balance.pdf
%
% Note that in a perfect world balance wants to be in the first
% column of the last page.
%
% If balance doesn't work for you, you can remove that and
% hard-code a column break into the bbl file right before you
% submit:
%
% http://stackoverflow.com/questions/2149854/how-to-manually-equalize-columns-
% in-an-ieee-paper-if-using-bibtex
%
% Or, just remove \balance and give up on balancing the last page.
%
\balance{}

\section{References Format}
Your references should be published materials accessible to the
public. Internal technical reports may be cited only if they are
easily accessible and may be obtained by any reader for a nominal
fee. Proprietary information may not be cited. Private communications
should be acknowledged in the main text, not referenced (e.g.,
[Golovchinsky, personal communication]). References must be the same
font size as other body text. References should be in alphabetical
order by last name of first author. Use a numbered list of references
at the end of the article, ordered alphabetically by last name of
first author, and referenced by numbers in brackets. For papers from
conference proceedings, include the title of the paper and the name of
the conference. Do not include the location of the conference or the
exact date; do include the page numbers if available. 

References should be in ACM citation format:
\url{http://www.acm.org/publications/submissions/latex_style}.  This
includes citations to Internet
resources~\cite{CHINOSAUR:venue,cavender:writing,psy:gangnam}
according to ACM format, although it is often appropriate to include
URLs directly in the text, as above. Example reference formatting for
individual journal articles~\cite{ethics}, articles in conference
proceedings~\cite{Klemmer:2002:WSC:503376.503378},
books~\cite{Schwartz:1995:GBF}, theses~\cite{sutherland:sketchpad},
book chapters~\cite{winner:politics}, an entire journal
issue~\cite{kaye:puc},
websites~\cite{acm_categories,cavender:writing},
tweets~\cite{CHINOSAUR:venue}, patents~\cite{heilig:sensorama}, 
games~\cite{supermetroid:snes}, and
online videos~\cite{psy:gangnam} is given here.  See the examples of
citations at the end of this document and in the accompanying
\texttt{BibTeX} document. This formatting is a edited version of the
format automatically generated by the ACM Digital Library
(\url{http://dl.acm.org}) as ``ACM Ref.'' DOI and/or URL links are
optional but encouraged as are full first names. Note that the
Hyperlink style used throughout this document uses blue links;
however, URLs in the references section may optionally appear in
black.

